Nonlinear Spectral Geometry Processing via the TV Transform

We introduce a novel computational framework for digital geometry processing, based upon the derivation of a nonlinear operator associated to the total variation functional. Such operator admits a generalized notion of spectral decomposition, yielding a sparse multiscale representation akin to Laplacian-based methods, while at the same time avoiding undesirable over-smoothing effects typical of such techniques. Our approach entails accurate, detail-preserving decomposition and manipulation of 3D shape geometry while taking an especially intuitive form: non-local semantic details are well separated into different bands, which can then be filtered and re-synthesized with a straightforward linear step. Our computational framework is flexible, can be applied to a variety of signals, and is easily adapted to different geometry representations, including triangle meshes and point clouds. We showcase our method throughout multiple applications in graphics, ranging from surface and signal denoising to detail transfer and cubic stylization.

==> Spectral TV (Copy)(3)/images/plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
%\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor1}{rgb}{1.00000,0.5882,0}%
%
\begin{tikzpicture}%
\begin{axis}[%
width=0.20\linewidth,
height=0.20\linewidth,
at={(-5.5cm,0)},
scale only axis,
ytick={0, 1},
yticklabels={0, 1},
xtick={0,1,3,5},
xticklabels={t=,1,3,5},
every x tick label/.append style={font=\color{black}, font=\footnotesize},
every y tick label/.append style={font=\color{black}, font=\tiny},
%xlabel={\footnotesize $t$},
ylabel={\footnotesize $u(t)$},
ylabel style={yshift=-0.25cm},
xlabel style={yshift=0.1cm},
xmin=0,
xmax=6,
ymin=-0.1,
ymax=1.2,
axis background/.style={fill=white}
]%
\addplot[forget plot, color=white!15!gray, dotted, line width=0.9pt] table[row sep=crcr] {%
0	0\\
6	0\\
};%
\addplot [color=mycolor1, line width=1.5pt, forget plot]%
  table[row sep=crcr]{%
0	1\\
0.00600600600600601	0.997998198198198\\
0.012012012012012	0.995996396396396\\
2.99099099099099	0.00310270270270274\\
2.996996996997	0.00110090090090087\\
3.003003003003	0\\
3.00900900900901	0\\
5.99399399399399	0\\
6	0\\
};%
\end{axis}%
\begin{axis}[%
width=0.20\linewidth,
height=0.20\linewidth,
at={(-2.75cm,0)},
%xlabel={ \footnotesize $t$},
ylabel={\footnotesize $\partial_t u(t)$},
ylabel style={yshift=-0.4cm},
ytick={-0.33, 0},
%ytick={-0.4, -0.3, -0.2, -0.1,    0,  0.1,  0.2},
yticklabels={-1/3,},
xtick={0,1,3,5},
xticklabels={t=,1,3,5},
every x tick label/.append style={font=\color{black}, font=\footnotesize},
xlabel style={yshift=0.05cm},
every y tick label/.append style={font=\color{black}, font=\tiny},
scale only axis,
xmin=0,
xmax=6,
ymin=-0.4,
ymax=0.2,
axis background/.style={fill=white}
]%
\addplot[forget plot, color=white!15!gray, dotted, line width=0.9pt] table[row sep=crcr] {%
0	0\\
6	0\\
};%
\addplot [color=mycolor1, line width=1.5pt, forget plot]%
  table[row sep=crcr]{%
0	-0.3333\\
0.00600600600600601	-0.3333\\
2.94294294294294	-0.3333\\
2.98498498498498	-0.3333\\
2.99099099099099	-0.3333\\
2.996996996997	-0.3333\\
3.003003003003	0\\
3.00900900900901	0\\
3.08108108108108	0\\
6	0\\
};%
\end{axis}%
\begin{axis}[%
width=0.20\linewidth,
height=0.20\linewidth,
%xlabel={ \footnotesize $t$},
ylabel={\footnotesize $\partial_{tt} u(t)$},
ylabel style={yshift=-0.25cm},
ytick={0, 1},
yticklabels={0, 1},
xtick={0,1,3,5},
xticklabels={t=,1,3,5},
every x tick label/.append style={font=\color{black}, font=\footnotesize},
xlabel style={yshift=0.05cm},
every y tick label/.append style={font=\color{black}, font=\tiny},
scale only axis,
xmin=0,
xmax=6,
ymin=-0.1,
ymax=1.2,
axis background/.style={fill=white}
]%
\addplot[ycomb, color=mycolor1, line width=1.5pt, mark=triangle, mark options={solid, mycolor1}, forget plot] table[row sep=crcr] {%
3.000300030003	1\\
};%
\addplot[forget plot, color=white!15!gray, dotted, line width=0.9pt] table[row sep=crcr] {%
0	0\\
6	0\\
};%
\node[right, align=left]
at (axis cs:3.2,1) {$\infty$};
\end{axis}%
\end{tikzpicture}%

==> Spectral TV (Copy)(3)/images/plottt.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(9.926in,0.596in)},
scale only axis,
xmin=0,
xmax=3,
ymin=0,
ymax=50,
xlabel=${t}$,
ylabel=$S(t)$,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	0\\
0.12	0\\
0.18	0\\
0.24	0\\
0.3	0\\
0.36	0\\
0.42	0\\
0.48	0\\
0.54	0\\
0.6	0\\
0.66	0\\
0.72	0\\
0.78	0\\
0.84	0\\
0.9	0\\
0.96	0\\
1.02	0\\
1.08	0\\
1.14	0\\
1.2	0\\
1.26	0\\
1.32	0\\
1.38	0\\
1.44	0\\
1.5	0\\
1.56	0\\
1.62	1.61326896783028\\
1.68	10.8664542039284\\
1.74	14.8863609697787\\
1.8	7.63896040637369\\
1.86	0.582923459225431\\
1.92	0\\
1.98	0\\
2.04	0\\
2.1	0\\
2.16	0\\
2.22	0\\
2.28	0\\
2.34	0\\
2.4	0\\
2.46	0\\
2.52	0\\
2.58	0\\
2.64	0\\
2.7	0\\
2.76	0\\
2.82	0\\
2.88	0\\
2.94	0\\
3	0\\
};
\end{axis}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(7.192in,0.596in)},
scale only axis,
xmin=0,
xmax=3,
ymin=0,
xlabel=${t}$,
ylabel=$S(t)$,
ymax=50,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	0\\
0.12	0\\
0.18	0\\
0.24	0\\
0.3	0\\
0.36	0\\
0.42	0\\
0.48	0\\
0.54	0\\
0.6	0\\
0.66	0\\
0.72	0\\
0.78	0\\
0.84	0\\
0.9	0\\
0.96	0\\
1.02	0\\
1.08	0\\
1.14	0\\
1.2	8.33793739352754\\
1.26	26.0897929810706\\
1.32	23.1722162857857\\
1.38	9.34430416355465\\
1.44	0\\
1.5	0\\
1.56	0\\
1.62	0\\
1.68	0\\
1.74	0\\
1.8	0\\
1.86	0\\
1.92	0\\
1.98	0\\
2.04	0\\
2.1	0\\
2.16	0\\
2.22	0\\
2.28	0\\
2.34	0\\
2.4	0\\
2.46	0\\
2.52	0\\
2.58	0\\
2.64	0\\
2.7	0\\
2.76	0\\
2.82	0\\
2.88	0\\
2.94	0\\
3	0\\
};
\end{axis}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(4.458in,0.596in)},
scale only axis,
xmin=0,
xlabel=${t}$,
ylabel=$S(t)$,
xmax=3,
ymin=0,
ymax=50,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	0\\
0.12	0\\
0.18	0\\
0.24	0\\
0.3	0\\
0.36	0\\
0.42	0\\
0.48	0\\
0.54	0\\
0.6	0\\
0.66	0\\
0.72	0\\
0.78	0\\
0.84	2.66365572617013\\
0.9	2.61165782452093\\
0.96	16.4075476525552\\
1.02	42.1779801784895\\
1.08	24.1490851884908\\
1.14	0\\
1.2	0\\
1.26	0\\
1.32	0\\
1.38	0\\
1.44	0\\
1.5	0\\
1.56	0\\
1.62	0\\
1.68	0\\
1.74	0\\
1.8	0\\
1.86	0\\
1.92	0\\
1.98	0\\
2.04	0\\
2.1	0\\
2.16	0\\
2.22	0\\
2.28	0\\
2.34	0\\
2.4	0\\
2.46	0\\
2.52	0\\
2.58	0\\
2.64	0\\
2.7	0\\
2.76	0\\
2.82	0\\
2.88	0\\
2.94	0\\
3	0\\
};
\end{axis}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(1.724in,0.596in)},
scale only axis,
xmin=0,
xmax=3,
ymin=0,
ymax=50,
xlabel=${t}$,
ylabel=$S(t)$,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	1\\
0.12	0.0354221564742846\\
0.18	0.0836880769716178\\
0.24	0.238515084607873\\
0.3	0.42369682621709\\
0.36	0.294829775280522\\
0.42	0.249205370448056\\
0.48	0.44619627845989\\
0.54	1.13388529065136\\
0.6	1.06936269974406\\
0.66	0.485097844802714\\
0.72	1.25885192956809\\
0.78	2.53080986474693\\
0.84	2.66365572617013\\
0.9	2.61165782452093\\
0.96	16.4075476525552\\
1.02	42.1779801784895\\
1.08	24.1490851884908\\
1.14	3.41464216740326\\
1.2	8.33793739352754\\
1.26	26.0897929810706\\
1.32	23.1722162857857\\
1.38	9.34430416355465\\
1.44	3.44171093089059\\
1.5	5.59118508341205\\
1.56	3.67877300861255\\
1.62	1.61326896783028\\
1.68	10.8664542039284\\
1.74	14.8863609697787\\
1.8	7.63896040637369\\
1.86	0.582923459225431\\
1.92	3.06471770053865\\
1.98	1.98939679353392\\
2.04	0.480183113497467\\
2.1	0.654214042504147\\
2.16	0.485439759045626\\
2.22	0.350683443571814\\
2.28	0.4174235136317\\
2.34	0.391300787515381\\
2.4	0.359935832863793\\
2.46	0.361220649315936\\
2.52	0.370039226720947\\
2.58	0.381070671319322\\
2.64	0.390812784387449\\
2.7	0.398571914814711\\
2.76	0.404053295448914\\
2.82	0.404623372677762\\
2.88	0.395091008572386\\
2.94	0.36869534607641\\
3	0.317572637938863\\
};
\end{axis}


\end{tikzpicture}%

==> Spectral TV (Copy)(3)/images/smeared.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mygray}{rgb}{0.50000,0.5,0.5}%
\definecolor{myblue}{rgb}{0.0804,0.5898,1}%
%
\begin{tikzpicture}
%
\begin{axis}[%
width=0.3\linewidth,
height=0.16\linewidth,
scale only axis,
xmin=-1,
xmax=1,
ymin=-0.1,
ymax=1.1,
axis line style={draw=none},
ticks=none,
legend style={legend cell align=left, align=left, draw=white!15!black}%
]%
\addplot [color=black, line width=1.6pt, forget plot]%
  table[row sep=crcr]{%
-1	0\\
-0.507537688442211	0\\
-0.49748743718593	1\\
0.49748743718593	1\\
0.507537688442211	0\\
1	0\\
};%
%
\end{axis}
%
\begin{axis}[%
width=0.3\linewidth,
height=0.16\linewidth,
at={(1.3cm,0)},
scale only axis,
xmin=-1,
xmax=1,
ymin=-0.1,
ymax=1.1,
axis line style={draw=none},
ticks=none,
legend style={legend cell align=left, align=left, draw=white!15!black}%
]%
\addplot [color=myblue, line width=1.6pt, forget plot]%
  table[row sep=crcr]{%
-1	0.0124316567871479\\
-0.979899497487437	0.0130917512766948\\
-0.959798994974874	0.0146526292205273\\
-0.939698492462312	0.0171633294536573\\
-0.919597989949749	0.0206993584857882\\
-0.899497487437186	0.0253605768668288\\
-0.879396984924623	0.0312682533993369\\
-0.85929648241206	0.0385612508652649\\
-0.839195979899497	0.047391324424003\\
-0.829145728643216	0.0524323585697029\\
-0.819095477386935	0.0579175464022208\\
-0.809045226130653	0.0638668667771738\\
-0.798994974874372	0.0702999180241104\\
-0.78894472361809	0.0772356828790115\\
-0.778894472361809	0.0846922871047318\\
-0.768844221105528	0.0926867539082068\\
-0.758793969849246	0.101234756512811\\
-0.748743718592965	0.110350371472953\\
-0.738693467336683	0.120045835518684\\
-0.728643216080402	0.130331308883783\\
-0.718592964824121	0.141214648195071\\
-0.708542713567839	0.152701192077583\\
-0.698492462311558	0.164793562654784\\
-0.678391959798995	0.190791635232835\\
-0.658291457286432	0.219169268976531\\
-0.638190954773869	0.249834462032695\\
-0.618090452261307	0.282640967168752\\
-0.597989949748744	0.317388599998267\\
-0.577889447236181	0.353825824698808\\
-0.557788944723618	0.391654619044215\\
-0.527638190954774	0.450260085944638\\
-0.447236180904523	0.608345380955784\\
-0.42713567839196	0.646174175301191\\
-0.407035175879397	0.682611400001732\\
-0.386934673366834	0.717359032831246\\
-0.366834170854272	0.750165537967304\\
-0.346733668341709	0.780830731023469\\
-0.326633165829146	0.809208364767164\\
-0.306532663316583	0.835206437345215\\
-0.296482412060302	0.847298807922416\\
-0.28643216080402	0.858785351804927\\
-0.276381909547739	0.869668691116216\\
-0.266331658291457	0.879954164481315\\
-0.256281407035176	0.889649628527045\\
-0.246231155778895	0.898765243487187\\
-0.236180904522613	0.907313246091791\\
-0.226130653266332	0.915307712895266\\
-0.21608040201005	0.922764317120986\\
-0.206030150753769	0.929700081975887\\
-0.195979899497488	0.936133133222824\\
-0.185929648241206	0.942082453597777\\
-0.175879396984925	0.947567641430295\\
-0.155778894472362	0.957225688506778\\
-0.135678391959799	0.965267656676309\\
-0.115577889447236	0.971849709455752\\
-0.0954773869346734	0.977117798921691\\
-0.0753768844221105	0.981202522974995\\
-0.0552763819095479	0.984214868075998\\
-0.035175879396985	0.986242833013094\\
-0.0150753768844221	0.987348904251816\\
0.00502512562814061	0.987568343212849\\
0.0251256281407035	0.986908248723303\\
0.0452261306532664	0.98534737077947\\
0.0653266331658291	0.98283667054634\\
0.085427135678392	0.979300641514209\\
0.105527638190955	0.974639423133169\\
0.125628140703518	0.968731746600661\\
0.14572864321608	0.961438749134733\\
0.165829145728643	0.952608675575995\\
0.175879396984925	0.947567641430295\\
0.185929648241206	0.942082453597777\\
0.195979899497488	0.936133133222824\\
0.206030150753769	0.929700081975887\\
0.21608040201005	0.922764317120986\\
0.226130653266332	0.915307712895266\\
0.236180904522613	0.907313246091791\\
0.246231155778895	0.898765243487188\\
0.256281407035176	0.889649628527045\\
0.266331658291457	0.879954164481315\\
0.276381909547739	0.869668691116216\\
0.28643216080402	0.858785351804928\\
0.296482412060302	0.847298807922416\\
0.306532663316583	0.835206437345215\\
0.326633165829146	0.809208364767164\\
0.346733668341709	0.780830731023469\\
0.366834170854271	0.750165537967304\\
0.386934673366834	0.717359032831247\\
0.407035175879397	0.682611400001732\\
0.42713567839196	0.646174175301191\\
0.447236180904523	0.608345380955784\\
0.477386934673367	0.54973991405536\\
0.557788944723618	0.391654619044215\\
0.577889447236181	0.353825824698808\\
0.597989949748744	0.317388599998267\\
0.618090452261306	0.282640967168752\\
0.638190954773869	0.249834462032695\\
0.658291457286432	0.21916926897653\\
0.678391959798995	0.190791635232835\\
0.698492462311558	0.164793562654784\\
0.708542713567839	0.152701192077583\\
0.71859296482412	0.141214648195071\\
0.728643216080402	0.130331308883783\\
0.738693467336683	0.120045835518684\\
0.748743718592965	0.110350371472953\\
0.758793969849246	0.101234756512811\\
0.768844221105528	0.0926867539082068\\
0.778894472361809	0.0846922871047318\\
0.78894472361809	0.0772356828790115\\
0.798994974874372	0.0702999180241104\\
0.809045226130653	0.0638668667771738\\
0.819095477386935	0.0579175464022208\\
0.829145728643216	0.0524323585697029\\
0.849246231155779	0.0427743114932193\\
0.869346733668342	0.0347323433236881\\
0.889447236180904	0.0281502905442457\\
0.909547738693467	0.022882201078307\\
0.92964824120603	0.0187974770250026\\
0.949748743718593	0.0157851319239992\\
0.969849246231156	0.013757166986903\\
0.989949748743719	0.0126510957481811\\
1	0.0124316567871479\\
};
%
\draw[-{Stealth[scale=1.1,inset=1.8pt,angle=90:10pt,color=gray,width=1.6mm,length=1.8mm]},semithick,gray] (-0.55,0.35) -- (0.55,0.35);
\draw[-{Stealth[scale=1.1,inset=1.8pt,angle=90:10pt,color=gray,width=1.6mm,length=1.8mm]},semithick,gray] (0.55,0.35) -- (-0.55,0.35);
%
\end{axis}
%
\begin{axis}[%
width=0.3\linewidth,
height=0.16\linewidth,
at={(2.6cm,0)},
scale only axis,
xmin=-1,
xmax=1,
ymin=-0.1,
ymax=1,
axis line style={draw=none},
ticks=none,
legend style={legend cell align=left, align=left, draw=white!15!black}%
]%
\addplot [color=myblue, line width=1.6pt, forget plot]%
  table[row sep=crcr]{%
-1	0\\
-0.507537688442211	0\\
-0.49748743718593	0.4\\
0.49748743718593	0.4\\
0.507537688442211	0\\
1	0\\
};%
\draw[-{Stealth[scale=1.1,inset=1.8pt,angle=90:10pt,color=gray,width=1.6mm,length=1.8mm]},semithick,gray] (0,1) -- (0,0.4);
%
\end{axis}
%
%
\end{tikzpicture}%

==> Spectral TV (Copy)(3)/images/treeplot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}
\begin{axis}[%
width=0.5\linewidth,
height=0.4\linewidth,
scale only axis,
xmajorgrids=true,
ymajorgrids=true,
every x tick label/.append style={font=\color{black}, font=\tiny},
every y tick label/.append style={font=\color{black}, font=\tiny},
ylabel style={yshift=-0.27cm},
ylabel style={xshift=-0.15cm},
xlabel style={yshift=0.17cm},
xmin=0,
xmax=3000,
xtick={0,1000,2000,3000},
xticklabels={0,1,2,3},
ytick={0,5000,10000},
yticklabels={0,,1},
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize Iteration ($\times 10^3$)},
ymin=0,
ymax=12000,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize TV energy},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={TV energy},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	8769.80567714888\\
3	8765.52060208535\\
6	8753.19870636316\\
10	8727.66111430032\\
15	8682.22208927593\\
21	8611.1679283053\\
30	8482.56228064604\\
47	8231.84418580489\\
73	7870.65280914336\\
91	7589.58614637022\\
117	7176.29431066304\\
127	7054.77059223718\\
140	6918.18548347215\\
175	6580.34393422045\\
188	6473.82821942617\\
215	6306.79157750887\\
226	6220.46841590536\\
236	6130.85882474641\\
249	6012.92683989099\\
260	5933.13604772369\\
266	5902.2598691463\\
286	5806.35904188635\\
296	5749.15997915603\\
314	5641.54918417365\\
345	5490.70561114222\\
355	5439.91918205179\\
367	5369.13998040854\\
387	5250.76948646463\\
399	5191.7422425948\\
414	5130.8492403156\\
426	5081.23042860648\\
463	4912.62785223861\\
471	4880.4776548674\\
481	4848.0619223422\\
494	4810.64507490459\\
508	4767.93847885284\\
519	4727.61524389073\\
550	4610.96550241506\\
557	4591.51193073569\\
567	4569.77743586156\\
591	4517.70972596239\\
609	4469.90139254135\\
628	4423.54846674126\\
648	4369.07492801303\\
677	4299.94310190137\\
682	4292.62112315639\\
691	4283.94144730481\\
701	4273.80408713521\\
720	4249.65352683481\\
732	4229.49252045151\\
748	4198.861309599\\
772	4146.23760459513\\
783	4122.15991394254\\
798	4092.73150577211\\
808	4068.01082555487\\
818	4038.35674322214\\
833	3987.40456568868\\
861	3879.95976558432\\
897	3745.50869204234\\
907	3716.44208462268\\
944	3627.41436387601\\
956	3591.75281018165\\
1000	3454.54209605356\\
1019	3403.79006415259\\
1039	3351.55111301218\\
1052	3312.02909201736\\
1071	3248.42261924547\\
1106	3128.77900846884\\
1113	3109.61331215802\\
1122	3091.27907023858\\
1136	3067.54776433203\\
1146	3053.55677953313\\
1155	3043.02032076248\\
1174	3022.79067289064\\
1209	2984.35951391489\\
1236	2945.70315345639\\
1259	2914.85047604769\\
1274	2894.34090030341\\
1293	2864.8364468102\\
1304	2848.9213213193\\
1321	2827.4305856946\\
1337	2807.47858652667\\
1350	2790.47637742014\\
1374	2765.0419230003\\
1384	2758.08015912145\\
1395	2752.17369725413\\
1403	2749.3970023681\\
1418	2744.74735744541\\
1426	2740.41932582834\\
1434	2733.93432471629\\
1442	2725.21744713767\\
1456	2706.47310609922\\
1480	2669.87699963885\\
1519	2605.4500996022\\
1548	2555.67374708552\\
1557	2544.5148062697\\
1566	2535.82702222485\\
1593	2514.54710694349\\
1602	2509.15521265019\\
1611	2505.73472131211\\
1619	2504.32144220168\\
1623	2505.15465380309\\
1636	2512.12597173624\\
1649	2517.96207204616\\
1670	2524.78404040088\\
1682	2526.34942406507\\
1697	2525.8474411031\\
1741	2521.55637672356\\
1761	2517.86695362734\\
1770	2513.39868070206\\
1779	2506.95550134922\\
1791	2495.90215132068\\
1830	2457.81727984579\\
1847	2441.31490656497\\
1867	2419.1369178171\\
1901	2381.00850024565\\
1921	2363.85352414888\\
1957	2335.53689928676\\
1963	2332.67572944614\\
1970	2331.17012275184\\
1979	2331.3986295762\\
2005	2333.98660748028\\
2024	2336.91933050283\\
2044	2340.14780063025\\
2065	2341.5292648391\\
2077	2340.46300584343\\
2090	2337.49786964739\\
2105	2331.76264729285\\
2166	2305.8037800657\\
2186	2300.36596434554\\
2222	2291.33805232033\\
2240	2283.77398112982\\
2256	2275.3927150391\\
2275	2262.87275449203\\
2297	2248.08989979396\\
2309	2242.15167615458\\
2332	2232.97669713028\\
2351	2224.77187911786\\
2364	2216.88876433548\\
2378	2206.06664404491\\
2404	2184.95588643737\\
2416	2177.29457953881\\
2463	2151.7182628464\\
2515	2127.27728830258\\
2535	2121.39195303474\\
2562	2114.55071084212\\
2578	2108.58621884492\\
2628	2087.94401443079\\
2651	2080.25598812873\\
2681	2071.09839012658\\
2701	2063.68138780557\\
2718	2055.58134480964\\
2745	2042.59158472335\\
2823	2008.67422338832\\
2839	1999.19300789203\\
2867	1982.38551697393\\
2889	1970.95692753235\\
2915	1959.59875683782\\
2951	1945.5664755403\\
2970	1939.80677396461\\
2991	1935.22020298349\\
2999	1933.84099657846\\
};
\addlegendentry{\footnotesize original}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	10282.0899593612\\
3	10240.8393369436\\
6	10125.466637058\\
10	9889.64524134536\\
16	9422.42888787062\\
28	8309.26230309407\\
39	7352.78915583833\\
50	6532.01735473021\\
62	5790.63661668084\\
80	4776.52254977473\\
89	4359.38492374121\\
96	4102.16732395772\\
107	3787.71059811782\\
118	3503.17106460966\\
126	3333.09489468827\\
131	3259.45367840321\\
135	3223.76848756533\\
138	3209.78813963662\\
141	3203.39382823318\\
154	3186.84011282525\\
162	3169.83785127707\\
180	3117.2572258599\\
184	3108.40364712658\\
191	3087.3562934762\\
198	3062.88621623496\\
204	3043.95045311897\\
224	2989.34078398757\\
231	2962.66956346121\\
238	2926.37221018255\\
253	2839.94192202754\\
267	2749.66071420537\\
279	2656.37391623455\\
307	2439.80630538242\\
322	2343.53041372188\\
330	2300.65424195822\\
340	2257.2994396219\\
349	2225.85037066919\\
358	2200.14958907804\\
368	2172.18233501462\\
383	2130.7338196834\\
390	2117.25996004967\\
431	2047.78242841884\\
437	2041.56194343109\\
450	2032.72105311146\\
476	2018.21626552898\\
483	2011.98182420321\\
489	2004.65188377867\\
496	1992.71960959904\\
504	1975.3168186967\\
522	1933.13963414107\\
545	1888.46892964927\\
556	1871.01303124894\\
566	1858.12849886948\\
580	1843.17403824954\\
588	1837.23855009064\\
599	1832.45144175262\\
614	1826.35197991301\\
641	1812.89249923677\\
653	1810.1313947828\\
664	1807.6828551932\\
672	1803.9879310629\\
681	1797.23946420362\\
702	1779.98251640605\\
712	1775.22782167409\\
723	1769.40903929834\\
733	1762.18339036431\\
744	1751.62346068541\\
771	1723.74524671412\\
782	1715.47151818146\\
793	1709.13617044166\\
802	1706.02023590914\\
815	1703.25767567192\\
880	1691.14126089583\\
911	1683.38975071214\\
929	1678.98366437674\\
953	1670.92914465903\\
974	1664.88040949725\\
1028	1649.71431451163\\
1073	1632.3601954541\\
1087	1629.11104696314\\
1102	1627.47999581991\\
1139	1624.27387252886\\
1172	1618.3197000878\\
1223	1606.99623914085\\
1251	1604.26034770985\\
1271	1603.74894491219\\
1305	1603.03117957847\\
1329	1601.1453996877\\
1355	1597.07549565886\\
1448	1580.68185897398\\
1480	1579.04357642985\\
1540	1576.05469636721\\
1584	1572.46436947919\\
1647	1567.64365305155\\
2037	1554.86004024981\\
2121	1553.58495724715\\
2214	1552.74730190819\\
2270	1551.51420469486\\
2407	1547.47944144937\\
2494	1544.81557924314\\
2559	1543.58033556663\\
2948	1541.57011783912\\
};
\addlegendentry{\footnotesize intrinsic triang}
\legend{}
\end{axis}
\end{tikzpicture}%

==> Spectral TV (Copy)(3)/sections/ack.tex <==
\begin{acks}
%
The authors gratefully acknowledge the anonymous reviewers for the thoughtful remarks, and Matteo Ottoni, Giacomo Nazzaro and Fabio Pellacini for the artistic and technical support. MF and ER are supported by the ERC Starting Grant No. 802554 (SPECGEO) and the MIUR under grant ``Dipartimenti di eccellenza 2018-2022'' of the Department of Computer Science of Sapienza University.
\end{acks}


==> Spectral TV (Copy)(3)/sections/apps.tex <==
\section{Applications}\label{sec:apps}
%
The TV spectral framework lends itself well to a variety of applications. In these, we follow the same computational procedure: 
%
\begin{enumerate}
\item Compute the forward TV transform of a given signal (possibly, the geometry itself);
\item Apply a filter to the resulting spectral components;
\item Compute the inverse TV transform.
\end{enumerate}



%We will now present some preliminary examples of applications of the proposed approach, which all fall under the same framework of applying a spectral filter in the TV spectral domain and then reconstruct the filtered signal in the spatial domain. 
%
%Spectral filtering is a classical task in linear spectral analysis, in which one aim to select frequencies in the spectral domain by applying filter operators to them, retaining or diminishing completely features at given scales in the reconstructed signal.

%This can be generalized in a straightforward manner to the nonlinear setting by applying the filter operator $I$ inside the inverse transform:

\noindent
Letting $u:\mathcal{M}\to\mathbb{R}^k$ be a $k$-channel signal on surface $\M$, $\phi_t$ be its spectral representation, and $I$ be a (possibly nonlinear) filtering operator, the filtered signal $\tilde{u}$ is computed as:
%
\begin{align}
   \tilde{u}= \int t I(\phi_t) dt \,.
\end{align}
%
Note that the above formula is meant to be generic, while in practice the type of TV regularization used to construct $\phi_t$ plays an important role as we shall see below.

We showcase our method on a range of relevant applications for graphics; for each application, we compare with other approaches from the state of the art to better position our method in terms of achievable quality. While these results are intended to demonstrate the flexibility of the framework, they are by no means exhaustive and could serve as a basis for follow-up work.


\begin{figure*}[t]
    \centering
    \begin{overpic}[width=\linewidth]{./images/figure_old01.png}
    \put(4.5,17){\footnotesize{Source}}
    \put(19.5,17){\footnotesize{\textbf{Ours}}}
    \put(30,17){\footnotesize{\cite{Zheng:2011}}}
    \put(44,17){\footnotesize{\cite{fleishman03}}}
    \put(60,17){\footnotesize{\cite{Sun:2007}}}
    \put(73.5,17){\footnotesize{\cite{Zhang:2015b}}}
    \put(88.5,17){\footnotesize{\cite{Jones:2003}}}
    \end{overpic}
    \caption{\label{fig:removal}{\em Top row:} Example of high-frequency detail removal, implemented as a \sout{simple} low-pass filter on the spectral TV representation of the source shape (leftmost). We get a ``rejuvenation'' effect on the face model (second column), and compare our solution with state-of-the-art approaches, specifically tailored for edge-preserving mesh filtering (third to fifth column). {\em Bottom row:} To better highlight the differences, we plot the mean curvature (clamped to $[-30 , 30]$ and color-coded, growing from blue to red) on the filtered surfaces. Our method is the most effective at removing wrinkles and obtains sharper feature lines compared to other approaches, which either tend to over-smooth or retain spurious vertex noise. A quantitative comparison \sout{over this data} is reported in Table~\ref{tab:curvEnergy}.}
\end{figure*}



%
\begin{figure}

%\linethickness{0.5mm} \color{blue}
%\put(0,0){\polygon(76 ,18)(76,12)(86,12)(86,18)}%(44,13.5)(22,13.5)(22,4.5)(0,4.5)}
 %   \end{overpic}
    \begin{overpic}[width=\linewidth]{./images/totem0.png}
    \put(44,-2){\footnotesize Laplacian}
    \put(77,-2){\footnotesize TV}
    \end{overpic}
  \caption{\label{fig:totem}Comparison between low-pass filtering of a source shape (left) \sout{in the Laplacian basis} using 300 Laplacian eigenfunctions (middle), and with our spectral TV representation using just \textbf{11 spectral components} out of 25 (right). The full shape has approximately $70k$ vertices. Laplacian-based smoothing correctly removes details, but also has a smoothing effect on the rest of the shape. In contrast, our approach correctly preserves the underlying structure.}
\end{figure}
%
\begin{table}
\resizebox{0.55\linewidth}{!}{
  \begin{tabular}{lc}
    \toprule
    \textbf{Method} & \textbf{TV Energy} \\
    \midrule
    Source & $43.412$ \\
     \textbf{Ours} & $\mathbf{26.55}$     \\
     \cite{Sun:2007} & $27.748$   \\
     \cite{Jones:2003} & $28.214$   \\
     \cite{Zhang:2015b} & $29.484$   \\
     \cite{fleishman03} & $31.918$   \\
     \cite{Zheng:2011} & $35.268$   \\
  \bottomrule
\end{tabular}
}
\caption{\label{tab:curvEnergy}Quantitative comparison between our TV spectral filtering method and the feature-preserving approaches from Figure~\ref{fig:removal}. For each method we report the TV energy of Eq.~\eqref{eq:soscurv}, which quantifies the amount of oscillations in the geometry after filtering; larger \textcolor{red}{values correspond to }\sout{numbers indicate the presence of} spurious noise.}
\end{table}

\subsection{Detail removal}
%
Perhaps the most straightforward application is the direct filtering of signals and geometric features living on the given surface. One such example is shown in Figure~\ref{fig:teaser}, where we apply a band-pass ``square window'' filter of the form:
%
\begin{align}
I_a^b(\phi_t) = \begin{cases}
\phi_t & t\in [a,b] \\
0 & \text{otherwise}\end{cases}
\end{align}
%
where $[a,b]$ is the range of time scales \sout{that are} left untouched by the filter; the normal field $\vec{n}$ is decomposed by applying Algorithm~\ref{PDHG} to  \sout{the isotropic total variation to} each component of $\vec{n}$ separately \textcolor{red}{and coupling the channels by projecting on the unit sphere at each step}. %\MM{OUT: While we did experiment with implementations of the total variation on the manifold $S^2$, we found the total variation of $\vec{n}$ in $\mathbb{R}^3$ along with iterative projections onto $S^2$ to yield favorable results (despite the resulting non-convexity).  }
% \MM{Did I describe this correctly, or is it "is decomposed by penalizing the sum of the $L_2$ norm of the stacked $x$-derivatives and the stacked $y$-derivatives"?} \textcolor{green}{(Marco) The signal is considered as a tri channel signal taking the norm over each signal separately. But during the minimization the channels are coupled as they are normalized at each step to remain on the sphere (approximately)} \MM{Ok, then I think my explanation (in terms the TV) is Ok, we just need to include the normalization}. 
The above filter relies upon one main property of the TV decomposition: The separation of geometric details into different spectral bands, \sout{which is} ensured by the underlying assumption that most interesting shapes have a sparse gradient.
%
\sout{Despite its very basic form,} This simple filter \sout{can} already provides \sout{very} high-quality selective suppression of semantic detail while preserving sharp geometric features. In  Figure~\ref{fig:removal} we compare to five other top performing methods from the literature,\sout{which are} specifically tailored to \sout{tackle} edge-preserving filtering, while we show a comparison with Laplacian-based filtering in Figure~\ref{fig:totem}.  %We show an additional example in Figure~\ref{fig:removal}, while in Figure~\ref{fig:totem} we compare with Laplacian-based filtering. 

\subsection{Detail transfer}
%
A remarkable application of the spectral TV framework is to transfer sharp geometric details between shapes. \sout{Let us be given} \textcolor{red}{Consider} two surfaces $\M,\mathcal{N}$ and a bijection $\pi:\mathcal{M}\to\mathcal{N}$ between them. Further, let $\phi_t$ and $\psi_t$ be the TV spectral representations of the normal fields on $\M$ and $\mathcal{N}$ respectively.
%
The idea is to transfer some components of $\phi_t$ to $\psi_t$ via $\pi$, and then compute the inverse transform of $\psi_t$ to obtain a new version of shape $\mathcal{N}$ with additional semantic details. 

%TODO: differenza with manifold-{\em valued} total variation

For this to work, recall that $\phi_t : \M\to\mathbb{R}^3$ is a vector field on $\M$ for any given $t\in\mathbb{R}_+$, and similarly for $\psi_t:\mathcal{N}\to\mathbb{R}^3$.
%
Therefore, we can transfer details from $\M$ to $\mathcal{N}$ by evaluating the integral:
%
\begin{align}
\tilde{u}(x) &= \int t (  \psi_t(x) + I_a^b(\phi_t)\circ\pi^{-1}(x) ) dt \label{eq:tx1}\\
&= u(x) + \int_a^b t ( \phi_t \circ \pi^{-1}(x) ) dt \,,
\end{align}
%
where $u$ is the original normal field on $\mathcal{N}$, $\tilde{u}$ is the newly synthesized normal field, and $I_a^b$ is a band-pass filter that selects the desired features to borrow from $\M$. The integral in Eq.~\eqref{eq:tx1} is a direct application of the reconstruction formula of Eq.~\eqref{eq:inv} to an additively updated spectral representation $\psi_t$. The key feature of this procedure is that, despite its simplicity, it enables a form of {\em selective} transfer of details. Importantly, the details must not be necessarily localized on the surface, as long as they are well localized in scale space.


In Figure~\ref{fig:transfer} we show an example of detail transfer.  In Figure~\ref{fig:coating} we compare our approach to the Laplacian-based detail transfer approach of \cite{Sorkine:2004}, where differences between Laplacian coordinates (i.e. differences between normals scaled by mean curvature) are transferred between shapes. For these tests, the map $\pi$ was computed using the method of \cite{zoomout} starting from $15$ hand-picked landmark correspondences.

\begin{figure}
    \centering
\begin{overpic}[width=0.9\linewidth]{./images/transfer.png}
\put(10,-3.5){\footnotesize{Source}}
\put(45,-3.5){\footnotesize{Target}}
\put(80.5,-3.5){\footnotesize{Result}}
\end{overpic}
    \caption{\label{fig:transfer}Example of detail transfer. The wrinkles on the source shape $\mathcal{X}$ (left) are captured with a high-pass filter in the spectral TV decomposition of $\mathcal{X}$, added to the spectral representation of the target (middle), and finally resynthesized (right). \sout{The clean separation between geometric features that is provided by} The TV decomposition allows to inject tiny {\em geometric} details into the target, without affecting the other bands (e.g., nose, mouth and ears are not affected by the transfer). Note that source and target shape do {\em not} have the same mesh connectivity, nor the same number of vertices.}
\end{figure}


\subsection{Stylization}\label{sec:Stylization}
%
We further exploit some basic properties of the TV flow for artistic rendition of 3D shapes. In particular, we show how with a proper choice of the \textcolor{red}{TV functional} \sout{total variation of $u\in BV(\M)$}, we get the desired effect of mimicking the stylistic features typical of voxel art. A similar effect of ``cubic stylization'' was achieved in \cite{huang2014} \sout{with the different intent of} for constructing polycube maps for texturing, and in \cite{cubic} for modelling purposes. These approaches minimize an as-rigid-as-possible deformation energy with $L_1$ regularization on the normal field. \sout{While our approach is different, it shares some generic properties with these techniques; namely, the modified shapes do not need any remeshing, hence they} \textcolor{red}{Similarly to these methods,} our modified meshes retain any attribute defined on the original shape (e.g. UV coordinates for textures). Further, since in our case the stylization is the result of an evolution process, this can be stopped at any time to attain the desired sharpness level.
A simple \sout{and immediate} way to get cubic stylization \textcolor{red}{is to consider} \sout{consists in considering} the $(x,y,z)$ coordinates as separate scalar functions regularized via the sum of anisotropic TV penalties. %The resulting projection of the dual variable in the $L^\infty$-ball (line 5 in Algorithm~\ref{PDHG}) induces a minimization of the oscillations with respect to the directions of the {\em global} reference frame; 
This causes the surface to flatten during the diffusion, and eventually shrink to a single point at convergence. Due to the strict dependence on the global reference frame, different orientations of the surface in $\mathbb{R}^3$ will give different results, as in \sout{the approaches of} \cite{huang2014,cubic}. %, as previously shown in Figure~\ref{fig:cat_cub}
%
\textcolor{red}{Shrinkage can be avoided by diffusing the normal vector field instead of the vertex positions.} \sout{A different perspective is provided again by considering the normal vector field as our input signal, this way constraining the normals (instead of the vertices) to align to the global coordinate axes.} %, with a notion of locality induced by the gradient defined on the surface. Exploiting this non local (w.r.t. $\mathcal{S}_2$ ) relation, we can obtain production quality results as shown in figures ( ref to figures).
 \sout{The main benefit of working with normals is that there will be no flattening or shrinkage of the reconstructed surface, since} \textcolor{red}{This way,} the flow only modifies the normal directions, and solving the screened Poisson equation~\eqref{eq:screened} approximately preserves the volume.
 %
 See Figures~\ref{fig:coating} and~\ref{fig:cubic} for some of our stylization examples.


%By applying a low pass filter in the spectral TV representation of the vertex coordinates, we can obtain a cubic geometric characterization of an arbitrary shape following the approach described in section 5.The idea of vertices alignment to the global axis can be exploited, to change the global reference frame and drive the minimization along different directions. One can go deeper and change the orientation of the  global reference frame to get the new geometric characterization for our shape.


\begin{figure}
    \centering
    \begin{overpic}[width=0.85\linewidth]{./images/detail_transf0.png}
\put(17,84){\footnotesize{Source}}
\put(9,-2.3){\footnotesize{\cite{Sorkine:2004}}}
\put(74,-2.3){\footnotesize \textbf{Ours}}
\put(73,84){\footnotesize{Target}}
\end{overpic}
    \caption{\label{fig:coating}{\em Replacing} the inscription from a source (top left) to a target model (top right), using Laplacian coating transfer \cite{Sorkine:2004} (bottom left), and our detail transfer approach (bottom right). The smoothing applied to the target causes the former approach to fail at preserving edges, while the transfer of high frequencies in the TV spectrum preserves them. The target model was obtained by applying our cubic stylization method of Section \ref{sec:Stylization} to the source model before superimposing the inscriptions.}
\end{figure}

\subsection{Denoising and enhancement}
%
% on point clouds + enhancement + localized operations
Finally, we demonstrate the application of the spectral TV framework to more classical tasks of geometry processing, namely surface denoising and enhancement. For these tests, we use both triangle meshes and point clouds.
\textcolor{red}{Once the spectral decomposition is computed, filtering and reconstruction can be performed in real time, as shown in the accompanying video.}

\sout{For these applications (as well as for detail removal above), once a spectral decomposition is performed, the filtering and reconstruction operations are especially efficient and can be carried out at interactive times. This is particularly useful in view of interactive applications, as shown in the accompanying video.}

\vspace{1ex}\noindent\textbf{Fairing.} \sout{Especially} When dealing with point clouds, denoising and fairing tasks are notoriously challenging due to the difficulty of distinguishing feature points from outlier noise. This confusion often requires pre-processing steps to localize sharp features and filter out the rest. In our setting, the edge-aware property of the TV functional allows us to automatically damp oscillations due to noise, while at the same time retaining the true details of the underlying surface.
%
We formulate denoising \sout{quite naturally,} as a simple low-pass filter in the spectral TV domain. The input signal is the normal field $\vec{n}:\M\to\mathbb{R}^3$; when $\M$ is discretized as a point cloud, normals can be estimated via total least squares \cite{mitra2003estimating}. See Figure~\ref{fig:denois} for an example of denoising of point clouds, where we compare with the recent bilateral filtering approach of \cite{Digne:2017}.


\begin{figure}
    \centering
    \begin{overpic}[width=0.85\linewidth]{./images/denosing_pcl0.png}
\put(14,90.5){\footnotesize{input 0.059}}
\put(14.5,-2.3){\footnotesize \textbf{Ours 0.022}}
\put(50,-2.3){\footnotesize{\cite{Digne:2017} 0.027}}
\put(67,90.5){\footnotesize{ground truth}}
\end{overpic}
    \caption{\label{fig:denois}The oriented point cloud on the top left (obtained by additive Gaussian noise on the vertex coordinates\sout{ of the ground truth}) is denoised by \sout{computing the spectral TV representation of its normal field, and} applying a low-pass filter \textcolor{red}{to the spectral TV representation of its normal field} (bottom left). On the bottom right we compare to Digne \sout{the recent bilateral filtering approach for point clouds of }\shortcite{Digne:2017}. At the top-right of each point cloud, we plot its normal field on the unit sphere. Points are color-coded according to their cosine similarity \textcolor{red}{(light to dark red, with values reported in the figure)} with the ground truth normals \sout{(small error is light red, large error is dark red)}\sout{ the ground truth normals are colored with} (in solid cyan)}
\end{figure}

\begin{figure*}
    \centering
    \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{./images/scene_final2.png}
    \end{overpic}
    \caption{\label{fig:cubic}Example of cubic stylization. The scene on the left is evolved along the {\em anisotropic} normal TV flow (i.e., each dimension of the normal vectors is treated as a separate scalar function, and these are regularized jointly via the sum of anisotropic TV penalties), which forces the normals to align with the global coordinate axes; the final result is shown on the right. \sout{The scene composition is for visualization purposes only;} Each shape was processed individually, and then placed in the scene.}
\end{figure*}
%\begin{figure}[h]
%    \centering
 %   \begin{overpic}[width=\linewidth]{./images/fig_denoising_pcl2.png}
%\put(10,-2.5){\footnotesize{input}}
%\put(33.5,-2.5){\footnotesize{ours}}
%\put(50.5,-2.5){\footnotesize{\cite{Digne:2017}}}
%\put(78.5,-2.5){\footnotesize{ground truth}}
%\end{overpic}
 %   \caption{\label{fig:denois}The oriented point cloud on the center left (obtained by adding Gaussian noise to the vertex coordinates of the ground truth) is denoised by computing the spectral TV representation of its normal field, and applying a low-pass filter to the representation. On the center right we compare to \cite{Digne:2017}. At the top-right of each point cloud, we plot its normal field on the unit sphere. Points are color-coded according to their cosine similarity with the ground truth normals (small error is light red, large error is dark red); the ground truth normals are colored with solid cyan.}
%\end{figure}




\vspace{1ex}\noindent\textbf{Enhancement.} While denoising can be seen as a suppression of high-frequency components in the spectral representation of $\vec{n}$, one can similarly obtain feature enhancement by {\em amplifying} those components; see Figure~\ref{fig:lion} for an example. Here we compare to the \sout{recent} gradient-based mesh processing approach of \cite{Chuang:2016:GPO}, which implements feature sharpening and smoothing \sout{(which are alternated in their pipeline) }by scaling the gradient of coordinate functions and solving for new coordinates via a Poisson equation. 
%
Conceptually, \sout{the main difference with our approach is in that} our spectral TV  representation allows more accurate control on specific features, since these are well separated in the spectrum; differently, the Laplacian-based approach adopted in \cite{Chuang:2016:GPO} encodes geometric features by spreading them out across the entire spectrum.

\begin{figure}
    \centering
\begin{overpic}[width=0.95\linewidth]{./images/fig_lion}
\put(23,84.5){\footnotesize{Source}}
\put(72,84.5){\footnotesize \textbf{Ours}}
\put(16,-2.5){\footnotesize{\cite{Chuang:2016:GPO}}}
\put(54,-2.5){\footnotesize{\cite{Chuang:2016:GPO}} w/ smoothing}
\end{overpic}
    \caption{\label{fig:lion}{\em Top row:} Spectral TV enhancement of a lion-shaped vase. Assigning a larger weight to the high-frequency spectral components has an effect of pronouncing the details of the 3D model, while preserving the sharp features. {\em Bottom row:} Comparison with \cite{Chuang:2016:GPO}. Their method comes in two variants. On the left, their direct sharpening results in a noisy mesh. On the right, feature enhancement is alternated with smoothing 3 times, at the cost of detail loss (e.g. around the whiskers).}

\end{figure}

\vspace{1ex}\noindent\textbf{Localized operations.} We conclude by mentioning that our framework also supports localized operations by means of masks defined over regions of interest, which could be useful in view of an interactive application for mesh editing (see the supplementary video). Let $R\subset\M$ be a region of $\M$, and let $I$ be an arbitrary spectral filter. Then, for a signal $u$ with spectral components $\phi_t$, localized spectral filtering can be carried out simply by evaluating:
%
\begin{align}
    \tilde{u}(x) = \rho(x) \int_\M t I(\phi_t(x))  dt\, + (1-\rho(x)) u(x),
\end{align}
%
where $\rho:\M\to [0,1]$ is an indicator function for $R$. %In Figure~\ref{fig:denois} we show an example of localized detail removal. \MM{Same figure reference as Fairing?}

%We can observe in figure \ref{fig:tvsmooth} how the total variation promotes piecewise constant solutions while preserving the details of the shape. This can be interpreted as Willmore flow variant which promotes sparsity. 

%\subsection{Denoising}
%Mesh denoising is a classical task in geometry processing to recover a good quality mesh from corrupted acquistion data. 

%Formally, the denoising problem reduces to solve the following optimization problem:\begin{align}
%    \min_u TV(u) + ||K u - u_0||_2^2
%\end{align}
%where $K$ is an operator, typically unknown, which encodes the noise applied to the signal. 


==> Spectral TV (Copy)(3)/sections/conclusion.tex <==
\section{Discussion and conclusions}
%
\sout{In this paper} We presented a new spectral processing framework for surface signals and 3D geometry\sout{(discretized as either triangle meshes or point clouds)}. The framework is based on ideas developed in the last decade within the nonlinear image processing community, but whose extension and application to geometric data \sout{and graphics tasks} have \sout{largely} been lagging behind to date. The main contribution of this paper is to show how these ideas can serve as valuable tools for computer graphics, and to relate the resulting observations and algorithms to more well known paradigms such as Laplacian-based spectral approaches and shape fairing via geometric flows.
%
Probably the most exciting aspect of the framework lies in its interpretability in terms of spectral components with an intuitive canonical ordering. Together with the \sout{discontinuity}\textcolor{red}{jump}-preserving property, \sout{the net result is} \textcolor{red}{one gets} the formation of frequency bands that tend to cluster together features with similar semantics. For example, the \sout{intertwining hair pattern} \textcolor{red}{hair strands} on a head model will be captured in a higher-frequency band than the ears; both will be captured sharply.
%
The general approach to mesh filtering that we described also retraces the steps of classical pipelines adopted in the linear case (transform -- filter -- resynthesize), making our nonlinear framework more accessible and of potentially broader impact.

%We have presented a new method based on a nonlinear operator derived from the total variation energy, which allows to analyze and decompose functions with discontinuities defined on manifolds. Through the study of the spectrum of this operator we showed how is possible to decompose and analyze signals at different scales, applying filters and transforming back in the original domain, just like in the linear case.
%Moreover we analyzed the evolution of the surface along the flow induced by the operator, obtaining strict relations with the mean curvature flow and the Willmore flow, and we showed how this operator is related to the standard Laplace Beltrami operator. Finally we showcased some possible applications of the proposed method showing that the spectral approach provides a unified framework for all of them.

\subsection{Limitations and future work}\label{sec:limitations}
%
\sout{Our method does have its limitations.} From a practical perspective, perhaps our weakest point is the need to define a schedule \sout{according to which} for the \sout{regularization} parameter $\alpha$ \sout{during the decomposition}, which determines the resolution of the spectral representation, \sout{in turn} influencing the design of filters. While in most cases an exact tuning \sout{of this parameter} is not required, it might be possible to define an adaptive scheme to automatically tune the scale of $\alpha$ to the feature landscape of the signal. Similarly, \sout{apart from the straightforward application of band-pass filters as we did in our tests,} a more sophisticated filter design to achieve complex effects is possible \sout{, but far from trivial} with \sout{To this end,} the adoption of learning-based techniques to predict task-specific filters \sout{may be highly beneficial}, as done \sout{for instance} in \cite{moeller2015learning} for image denoising. More generally, the integration \sout{this framework} within geometric deep learning pipelines is a promising direction that we are eager to pursue.
%As stressed in previous sections the regularization parameter $\alpha$ has a key role in the spectral representation as it is proportional to time of diffusion along the TV flow. While ideally one would choose a non uniform interval of values for alpha such to capture and separate all the spectral features, at the current stage there are no guarantees on how to choose these values apriori of the signal decomposition.
%The  most  limiting  aspect of the proposed spectral approach is that it is not still clear if is possible to build a basis from the spectrum of the $\partial TV$ operator, although its existence has been proven in theory (see \cite{le:2006}). This restricts the decomposition to be signal dependent.
%\subsection{Future perspectives}
%The ideas explored in the development of this paper open many interesting paths to explore in future works. 
We also anticipate that the study of the more general $p$-Laplacian operator on surfaces \sout{will likely} \textcolor{red}{might} lead to a richer class of algorithms for geometry processing. One promising idea is to define the operator adaptively, \sout{by} selecting a value for $p$ depending, \sout{on certain geometric properties of the shape} e.g., on curvature. Finally, a more in-depth analysis of the normal TV flow as a robust alternative for mesh fairing is essential, due to its \sout{remarkable} feature preservation properties and its \sout{strict} connection to other \sout{common} geometric flows.

%A first direction would be the one of studying the spectrum of the $p$-Laplacian operator on surfaces, defining an operator which adapts $p$ to the geometry of the domain. 

%Another key point would be the one to develop strategies to find the optimal values for the regularization parameter $\alpha$, to best separate scale features of a signal depending on the given task one has to accomplish.


==> Spectral TV (Copy)(3)/sections/flow.tex <==
\section{Geometric TV flow}
%
\sout{In this Section,} We now study the evolution of the surface $\M$ \sout{itself} along the TV flow.
%
A direct way to do this is to evolve the $(x,y,z)$ vertex coordinates of $\M$; the same approach is also used to define, e.g., the mean curvature flow (MCF) and its variants \cite{Taubin:1995,Desbrun:1999,kazhdan2012can}. % , considered as a multichannel signal in which discontinuities and sharp changes represent the details of the shape.
This approach, however, gives rise to two main issues.

%Computing the TV transform of this signal we obtain a multiscale representation of a shape, where filtering high to low frequency components correspond to diffuse the surface along the TV flow.

First, diffusing the vertex coordinates naturally affects the metric of $\M$ at each diffusion step; this, in turn, modifies the functional $TV(f)=\int_\M \|\nabla_\M f\|$, since the integration domain $\M$ and the attached intrinsic operators now vary along the flow. % This brings major challenges in the integration due to the change of the metric of the initial embedding along the flow, with respect to which the gradient and divergence operators are defined.
%
 Recomputing the metric-dependent operators at each iteration of the algorithm is a possible solution, but can be highly inefficient.
 
 %(also because a single iteration of the algorithm does not affect the metric significantly).

%To solve the problem one could take advantage of the variable splitting in the primal dual formulation and precondition the gradient and  divergence operators, while  balancing the change in the metric by dynamically adapting the area weights.

Secondly, one must take care of the choice of the TV regularization for $(x,y,z)$. In fact, for $f$ being the coordinate function on the manifold, $\nabla f(x)$ becomes a tensor for which a suitable norm $\|\nabla f(x)\|$ in the integral of the total variation needs to be defined. Depending on such a choice one can encourage different types of collaborative gradient sparsities \cite{Duran16}. For example, by choosing a fully anisotropic TV (i.e. summing the absolute value of all entries in $\nabla f(x)$), the transform will be orientation-dependent: the diffused vertex coordinates will tend to align to the global reference frame of $\mathbb{R}^3$, giving different results depending on the orientation of the initial shape; see Figure~\ref{fig:cats} for examples. While this latter point can be exploited for certain stylization tasks (as we show in Section~\ref{sec:apps}), it might be an undesirable effect in many other applications.
%


\begin{figure}
\centering
      \includegraphics[width=\linewidth]{images/cats.png}
  \vspace*{-0.7cm}
  \caption{\label{fig:cats}Diffusing vertex coordinates on the cat model. An anisotropic TV penalty will promote piecewise-flat solutions, where oscillations are minimized along the coordinate axes. Therefore, one gets different results by rotating the global reference frame; for the source model on the left, we show solutions \sout{of the flow} under two different axis rotations (middle and right respectively).}
\end{figure}

%Nonetheless this provides us a way to act on details of the shape at different scales the oscillations along the direction spanned by the three reference axis, as we can observe in figure \ref{fig:cat_cub}. 

\begin{figure}
  \centering
\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.95\linewidth]{images/clusters.png}
\end{overpic}
  \caption{\label{fig:gargoyle}Our flow induces the formation of clusters in the normal field. The top row shows the original surface, the bottom row is the filtered result. {\em Middle}: the local density of the Gauss map (heatmap growing from white to red) illustrates the formation of clusters in normal space. {\em Right}: the coverage of $\mathcal{S}^2$ \textcolor{red}{(front and back sides visualized)} shows that the diffused normals are less spread across the sphere than in the original surface.\sout{; the other side of the sphere is visualized here for a more complete picture.}}
\end{figure}

%\MM{introduce TV on vector valued functions and discuss possible choices for the norm. For a detailed discussion in the Euclidean space see \cite{Duran16}. sum from 1 to k of per-channel tv.}

\sout{Due to the aforementioned problem of changing meshes, we instead propose a different type of geometric flow as we will discuss in the next section.}

\subsection{Normal TV flow}

In this paper we advocate the use of normal fields for encoding the geometry. This choice has three main benefits: (1) the domain upon which the operators are defined remains fixed throughout the flow; (2) using normals endows us with {\em rotation invariance}; and (3) we get interesting connections with other existing flows.
%
Normal fields in connection with the TV functional have been considered before, e.g. in \cite{Zhang:2015,Zhong:2018}. However, these approaches do not consider or analyze the geometric flow as we do here, and do not provide a natural and interpretable multiscale decomposition.

%
\setlength{\columnsep}{7pt}
\setlength{\intextsep}{1pt}
\begin{wrapfigure}[5]{r}{0.40\linewidth}
\begin{center}
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=1.0\linewidth]{./images/buns.png}
\put(49.5,35){\footnotesize $\Gamma$}
\put(46,29){\footnotesize $\longrightarrow$}
\end{overpic}
\end{center}
\end{wrapfigure}
%
%In order to define a {\em rotation-invariant} flow, i.e. which does not depend on the orientation of the surface immersion in $\mathbb{R}^3$, 
Our input signal is the normal vector field $\vec{n}_0$ over $\M$. The field $\vec{n}_0$ is identified by the image of the Gauss map $\Gamma : \M \rightarrow \mathcal{S}^2$, mapping points on the surface to points on the unit $2$-sphere (see inset).
%
The corresponding time continuous flow is:
%
\begin{align}\label{eq:npde}
    \begin{cases}
    \frac{\partial \Gamma}{\partial t}= ~\mathrm{div}_{S} \left(\frac{ d\Gamma }{\|d\Gamma\|}\right) &  \text{in  } \mathcal{S}^2,\\
    \Gamma(0,x) = \vec{n}_0 \,,
    \end{cases}
 \end{align}
 %
 where $d \Gamma$ is the differential of the Gauss map \sout{(aka shape operator),} and $\mathrm{div}_S$ is defined with the metric of $\M$, but applied to tangent fields on $\mathcal{S}^2$.
%
By diffusing normals according to Eq.~\eqref{eq:npde}, \sout{the domain $\M$ stays fixed throughout the entire flow (thus, its metric does not need to be updated at each iteration), while} the point distribution over $\mathcal{S}^2$ changes to form well-separated clusters. Intuitively, the flow tends to align the directions of normal vectors to favor piecewise-constant solutions; see Figure~\ref{fig:gargoyle} for an example. \sout{of normal re-distribution induced by the flow;} To obtain the filtered embedding for $\M$, the diffused normal field is integrated as described further in this section.

\sout{
%\begin{remark}
The clustering induced by the normal TV flow is {\em not} equivalent to running a clustering algorithm in normal space, since the flow is defined w.r.t. the metric on the {\em original} surface $\M$. A simple clustering of nearby normals would instead use the metric of $\mathcal{S}^2$.
%\end{remark}
}

%Since the surface $\M$ is fixed, the TV flow algorithm can be applied as-is without updating the metric. Further, since , the flow is invariant to global rotations of $\M$.


%\begin{figure}[t]
  %\centering
  %\begin{overpic}[percent,width=\linewidth]{buns.png}
  %\put(10,30){$\M$}
  %\put(55,30){$\mathcal{S}_2$}
    %\put(100,5){$\mathcal{S}_2$}
  %\includegraphics[width=\linewidth]{bunnygauss.jpg}
   %\end{overpic}
  %\caption{Gauss Map representation of the bunny model  on the sphere} \label{fig:bun_gauss}
%\end{figure}

%Depending on the regularization parameter $\alpha$, 

%\textcolor{red}{questo mettiamolo nella caption di una figura in cui confrontiamo normal tv flow con vertex flow e magari con clustering su s2:} The solution of the normal TV flow will tend to align the directions of normal vectors at different scales, favoring piecewise-constant solutions.

Interpreting this approach from a differential geometric perspective provides us with a useful characterization of the normal TV flow in terms of surface curvature. In particular, the TV functional for the normal field $\vec{n}$ reads:
%
\begin{align}\label{eq:soscurv}
    TV(\vec{n})=
    %\int_\M \|\nabla_{\M} \vec{n}\|=
    \int_{\M} \| d \Gamma (x) \| dx=
    %\int_{\M} | S_p  | = 
    \int_\M \hspace{-0.05cm} \sqrt{k_1^2 + k_2^2} \, dx\,,
\end{align}
%
where  %, aka the shape operator $\mathcal{S}_p:\mathcal{T}_p\M \rightarrow \mathcal{T}_p \M$ which maps vectors from the tangent space on the surface to the tangent space on the sphere, and 
 %encodes curvature information of the surface. It is expressible as a $2x2$ matrix %(also called II fundamental form )
 %whose eigenvalues are the principal curvatures $k_1, k_2$. 
 $k_1,k_2$ are the principal curvatures at each point.
 %
 The last equality follows from the fact that $k_1,k_2$ are the eigenvalues of $d\Gamma$.
 
 %The determinant of this matrix is the Gaussian curvature and its half trace is the mean curvature. The total variation functional in this case corresponds to
 
 %\footnote{The third equality is justified by the fact that $|S_p|^2= (S b1 )^T(S b1 ) +(S b2 )^T(S b2 )$, where b1,b2 are basis vectors of the tangent space at $p$. Choosing the principal directions $K_1, K_2$ as basis vectors, we get the square root of the sum of squares of principal curvatures. }: 
 
As we show below, the final expression in Eq.~\eqref{eq:soscurv} resembles the functional related to other known flows in the literature. We also see from the same expression that the TV energy of the normal field does {\em not} depend on the orientation of the normals in $\mathbb{R}^3$; therefore, the resulting flow is invariant to global rotations of $\M$. 

%Since we have changed the optimization domain to the sphere now the integrand is no more dependent on the domain.

\vspace{1ex}\noindent\textbf{Implementation.}
%
By working with normal fields $\vec{n}$ we are moving to manifold-{\em valued} functions (the manifold being the unit sphere).
%, for which a TV functional must be properly defined \cite{lellmann13}.
 %For simplicity, 
 In our tests we treat each $\vec{n}(x)$ as an element of $\mathbb{R}^3$, and add a normalization step projecting $\vec{n}(x)$ back onto $\mathcal{S}^2$ at each iteration.

%\MM{This is something I'd like to understand in more detail: The total variation of a manifold-valued function needs some considerations for how to define gardients, see \cite{lellmann13}. Or did you treat $\vec{n}$ as an element of $\mathbb{R}^3$ rather than $\mathcal{S}^2$?}

In the discrete setting, the normal vector field $\mathbf{n}\in\mathbb{R}^{|F|\times 3}$ is constant within each triangle. %To process it in the proposed framework one has two main choices: either to approximate the signal over vertices  and use the classical gradient definition or to change the gradient definition. We opt for the latter since the former, while simpler, may introduce artifacts in the reconstruction of vertex coordinates due to the approximation.
 Its gradient (needed in Algorithm~\ref{PDHG}, line 5) is understood as the channel-wise jump discontinuity over each edge in each triangle, and the associated discrete operator can be assembled as a $|E| \times |F| $ matrix; see Appendix~\ref{sec:edgegrad} for details.
 
 \begin{figure}[t]
    \centering
\begin{overpic}[width=\linewidth]{images/dogs.png}
\put(4.7,6.4){\footnotesize source}
\end{overpic}
\caption{Comparison between MCF (top row) and normal TV flow (bottom row) on a 1D closed contour \sout{depicting} of a dog. The circles visualize the image of the Gauss map on $\mathcal{S}^1$ for each shape; the color code is defined as on the source shape (leftmost column). The MCF equally spreads the normals, eventually converging to a circle, while the TV flow forms well-separated clusters \sout{of normals (in this example,} (\sout{concentrated around} the 5 points on the circle), converging to a piecewise-flat shape.}
\label{fig:1dflow}
\end{figure}

\vspace{1ex}\noindent\textbf{Recovering vertex positions.}
%
To recover a new embedding from the filtered normals $\mathbf{n}$, we follow \sout{the approach of} \cite{Prada:2015}\sout{ and solve the optimization problem}:
%
\begin{align}\label{eq:poisson}
        \min_{\mathbf{v} \in \mathbb{R}^{|V|\times 3}} \| \mathbf{G} \mathbf{v} - \mathbf{w}\|_F^2 + \epsilon \|\mathbf{v}-\mathbf{v}_0\|_F^2\,,
\end{align}
%
where $\mathbf{v}_0$ are the old vertex coordinates, and $\mathbf{w}=\mathbf{Gv}_0- \langle \mathbf{Gv}_0,\mathbf{n} \rangle_r \odot \mathbf{n}$ is the orthogonal component of $\mathbf{G} \mathbf{v}_0$ with respect to $\mathbf{n}$ ($\langle\cdot,\cdot\rangle_r$ and $\odot$ operate row-wise).
%
% $\mathbf{w}=\mathbf{Gv}_0 - \mathrm{diag}((\mathbf{Gv}_0) \mathbf{n}^\top)\mathbf{n}$ 
%
Eq.~\eqref{eq:poisson} seeks the set of vertices whose gradient matches the vector field $\mathbf{w}$, while at the same time staying close to the initial vertices. \sout{The first term is inspired by the gradient-based energy of Yu:2004.} In our tests we set $\epsilon=10^{-4}$ to allow large deviations from the initial shape.
Solving Eq.~\eqref{eq:poisson} boils down to solving a screened Poisson equation, giving the sparse linear system:
%
\begin{align}\label{eq:screened}
        \mathbf{v}=(\epsilon \mathbf{A}- \mathbf{L})^{-1}( \epsilon \mathbf{A} \mathbf{v}_0 - \mathbf{D} \mathbf{w})\,.
\end{align}
%
Here, $\mathbf{L}=-\mathbf{DG}$ corresponds to the standard linear FEM discretization of the Laplace-Beltrami operator.




\subsection{Related curvature flows}
%
\sout{Here} We compare our \sout{normal TV} flow to other geometric flows used in graphics.

\vspace{1ex}\noindent\textbf{Mean curvature flow.}
%
The \textcolor{red}{normal} TV flow is closely related to the MCF, which describes the evolution of a surface under the minimization of the area functional (membrane energy):
%
\begin{align} \label{eq:areafnctl}
    E_A(u) = \int_\M dx \,,
\end{align}
%
%where $da = \sqrt{det g} $ is the area element and
where $u$ is now the $(x,y,z)$ embedding in $\mathbb{R}^3$ of the surface $\M$, and we assume $\M$ has no boundary. The relation to our flow emerges by approximating the membrane energy with the Dirichlet energy $E_A(u)\propto D(u)=\frac{1}{2}\int_\M \| \nabla u \|^2$, whose gradient flow is the PDE:
%
\begin{align}
    \frac{\partial u}{\partial t} = \Delta u \,.
\end{align}
%
Compared to Eq.~\eqref{eq:pde}, this PDE uses the linear operator $\Delta=\mathrm{div}\nabla$ instead of the nonlinear operator $\mathrm{div}\frac{\nabla}{\|\nabla\|}$. 

Denoting with $H = \frac{k_1 + k_2}{2}$ the mean curvature, and observing that $\Delta u = 2H \vec{n}$, the above PDE corresponds to 
%\begin{align}
 %   \frac{\partial f}{\partial t} = -H n 
%\end{align}
  surface motion in the normal direction, with speed proportional to curvature $H$. Critical points of the functional are minimal surfaces, which for genus-0 \textcolor{red}{convex} shapes correspond to spheres.
  
In comparison, surface evolution along the normal TV flow collapses the surface to a flat shape, with the direction of motion perpendicular to the level sets of the normal vector field $\vec{n}$.
%
By looking at the effect of the flow on $\vec{n}$, the key difference is that the MCF tends to move points on $\mathcal{S}^2$ so as to keep them equally spaced, while the normal TV flow generates well-separated point clusters. We illustrate the comparison in 2D in Figure~\ref{fig:1dflow}; an example of our feature-preserving flow in 3D is given in Figure~\ref{fig:bimba}.


\begin{figure}
\begin{overpic}[width=\linewidth]{images/bimba}  
\end{overpic}
    \caption{\label{fig:bimba}Normal TV flow on the bimba\sout{ model}.  Sharp geometric features get smoothed in a ``vertical'' fashion, preserving the overall structure. For example, the chin and pony tail maintain their shape throughout, while the braid and nose slowly disappear without affecting the neighboring geometry.}
\end{figure}



\vspace{1ex}\noindent\textbf{Willmore flow.}
%
Perhaps more interestingly, we observe that our functional $TV(\vec{n})$ resembles the Willmore (or thin plate) energy \cite{Bobenko:2005:}, \sout{which is} a higher-order version of the area functional, \sout{and is} defined as:
%
\begin{align}\label{eq:will}
    E_W(u) = \int_\M H^2 dx = \int_\M (k_1^2 + k_2^2) \, dx - \cancel{2\pi\chi(\M)} \,,
\end{align}
%
where again $u$ encodes the coordinate functions in $\mathbb{R}^3$. The last term is the constant Euler characteristic of $\M$, and thus it does not affect the flow.
%
Compared to Eq.~\eqref{eq:soscurv}, we see that the integrand only changes by a square root operation. In this sense, we interpret the normal TV flow as a sparsity-promoting variant (in the normal domain) of the Willmore flow. 

The linearization of Eq.~\eqref{eq:will} leads to a fourth-order bi-Laplacian diffusion equation:
%
\begin{align}
     \frac{\partial u}{\partial t} = \Delta^2 u \,.
\end{align}
%
Our problem also involves a fourth-order PDE with respect to the coordinates; however, it is hard to solve directly due to the nonlinearity of our operator. By phrasing the PDE in terms of the normals instead of the coordinates, we decouple the problem: first we integrate the TV flow in the space of normals, which corresponds to the {\em second}-order PDE of Eq.~\eqref{eq:npde}, and then we integrate again to recover the vertex coordinates via the screened Poisson equation. %In particular, step (1) only involves first-order operators ($\mathrm{div}$ and $\nabla$).


\begin{table}
  \begin{tabular}{lll}
    \toprule
    \textbf{Flow} & \textbf{Functional} & \textbf{PDE}\\
    \midrule
    MCF & $E_A(u) = \int dx $& $    \frac{\partial u}{\partial t} = \Delta u$ \\
    Willmore & $E_W(u) =\int (k_1^2 + k_2^2)$ & $   \frac{\partial u}{\partial t} = \Delta^2 u $
    \\
    TV & $E_{TV}(\vec{n}) = \int \hspace{-0.05cm} \sqrt{k_1^2 + k_2^2} \, dx$ & $\frac{\partial \Gamma}{\partial t}= ~\mathrm{div}_S \left(\frac{d\Gamma}{\|d\Gamma\|}\right)$\\
  \bottomrule
\end{tabular}
\caption{\label{tab:flows}Comparison between MCF, Willmore, and our normal TV flow in terms of functional involved and the associated PDE.}
\end{table}



\begin{figure}
\begin{overpic}[width=\linewidth]{images/bunny_flow}  
\put(-1.5,6){\rotatebox{90}{\footnotesize TV}}
\put(-1.5,21){\rotatebox{90}{\footnotesize Willmore}}
\put(-1.5,43){\rotatebox{90}{\footnotesize MCF}}
\put(8,-2){
\begin{tikzpicture}
\draw[->,line width=0.15mm](0,0) -- (1,0);
\end{tikzpicture}}
 \put(80.5,5){
\begin{tikzpicture}
\draw[-,line width=0.15mm](0,0) -- (0,3.65);
\end{tikzpicture}}
% \put(81,56){
%\begin{tikzpicture}
%\draw[-,line width=0.15mm](0,0) -- (1.5,0);
%\end{tikzpicture}}
\put(84,-2){\footnotesize convergence}
\end{overpic}
    \caption{Evolution of the bunny surface along different geometric flows. Top to bottom: conformalized mean curvature flow \cite{kazhdan2012can}, conformal Willmore flow \cite{Crane:2013:RFC}, and our normal TV flow. The TV flow differs from the others as it preserves the underlying structure, and details are removed gradually. At convergence, we get a flat surface since the image of the Gauss map is clustered into a single point on $\mathcal{S}^2$.}
    \label{fig:3dflow}
\end{figure}


%
In Table~\ref{tab:flows} we summarize the three flows\sout{ to better highlight their analogies}. A qualitative comparison is shown in Figure~\ref{fig:3dflow}, \sout{for a fair comparison,} where we use stable variants of the existing flows that prevent \sout{numerical} singularities.
%
%Further, in Figure~\ref{fig:bimba} we show another example of our flow, on a shape with sharper features compared to the bunny.


%\begin{figure}[bth]
%  \centering
%  \begin{overpic}[scale=0.24]{images/dogs2.png}
%  \put(11,35){\footnotesize Original}
%  \put(43,35){\footnotesize TV flow}
%  \put(81,35){\footnotesize MC flow}
%  \put(-5,55){$\mathbb{R}^2$}
%  \put(-5,15){$\mathcal{S}^1$}
%    \end{overpic}
%    \begin{overpic}[scale=0.24]{images/dogs2.png}
%  \put(11,35){\footnotesize Original}
%  \put(43,35){\footnotesize TV flow}
%  \put(81,35){\footnotesize MC flow}
%  \put(-5,55){$\mathbb{R}^2$}
%  \put(-5,15){$\mathcal{S}^1$}
%    \end{overpic}
%  \caption{For a flat shape (left), we compare the TV flow of the normals (center) and MCF (right), representing the 1D surface in $\mathbb{R}^2$ (top row) and its normal vector field on $\mathcal{S}_1$ (bottom row)}
 % \label{fig:1dflow}
%\end{figure}




\subsection{The p-Laplacian operator}
%
We remark here that both the Laplace-Beltrami operator $\Delta_\M$ and the \sout{nonlinear TV} subdifferential $\partial TV$ explored in this paper are special cases of a more general parametric operator, the $p$-Laplacian \cite{Lindqvist:2006}:
%
\begin{align}
    \Delta_p = \mathrm{div} (\|\nabla\|^{(p-2)} \nabla  )\,,
\end{align}
with the associated $p$-Dirichlet energy:
\begin{align}
    E_p(u) = \frac{1}{p}\int_\M \|\nabla u\|^p dx \,.
\end{align}
%
In particular, the $p$-Dirichlet energy with $p=1$ corresponds to the TV functional, while for $p=2$ we retrieve the standard Dirichlet energy.
%
By studying the solution for the evolution along the $p$-Laplacian flow of a unit ball, we observe convergence to a cube for $p=1$ (TV), to a sphere for $p=2$ (Dirichlet energy) and to an octahedron for $p \gg 2$, which is a consistent behavior with the definition of $p$-norms  (see Figure~\ref{fig:plaplacian}).
%
From the example we see clearly that the TV flow tends to piecewise-flat solutions, and further observe that other $p$-Laplacian flows carry other properties that may be worth investigating in the future. We refer to \cite{Buehler09} for a discussion on the eigenvectors of the $p$-Laplacian and to \cite{Cohen19} for an approach defining a $p$-Laplacian-based spectral decomposition in Euclidean spaces. 

%\textcolor{green}{si potrebbe aggiugere qualcosa forse commentando il cambio di funzione di base (da costante a tratti per p=1 a smooth per p=2, facendo vedere un'immagine).}

\begin{figure}
    \centering
   \begin{overpic}[width=\linewidth,scale=0.25]{sphere.png}
    \put(9,17){\footnotesize $p=2$}  
    \put(37,17){\footnotesize$p=1$}  
    \put(62,17){\footnotesize$p=5$}  
    \put(89,17){\footnotesize$p=1.5$}
    %
    \put(9.5,-3){\footnotesize MCF}
    \put(38.5,-3){\footnotesize TV}
    \end{overpic}
    \caption{Evolution of \textcolor{red}{the vertex coordinates} of the unit $L_2$ sphere along \sout{different} $p$-Laplacian flows, for different values of \sout{parameter} $p$. \sout{The input signal here are the vertex coordinates $(x,y,z)$;} The flows are simulated with the explicit Euler method. For $p=2$ the sphere remains a sphere, while it becomes a piecewise-flat surface with the TV flow ($p=1$).}
    \label{fig:plaplacian}
\end{figure}

==> Spectral TV (Copy)(3)/sections/implementation.tex <==
\section{Implementation}\label{sec:impl}
%
%\textcolor{red}{dovremmo pensare di nuovo se spostare in Appendix o no, il paper potrebbe risultare pesante da leggere}

We implemented the framework in Matlab 2019a, and ran all the experiments on an Intel i7-4558U  CPU with 16 GB RAM. \sout{The code will be made publicly available upon acceptance.}
%
A discussion on runtime performance \sout{together with a runtime table for our experiments are} is provided in Appendix~\ref{sec:runtime}.

%\MM{We discretize all shapes by triangles and use an operator that computes one gradient vector per triangle to discretize the total variation. The resulting optimization problem (similar to \eqref{eq:dtv}) that we need to minimize iteratively to compute the flow is solved via the primal-dual hybrid gradient method \cite{chambolle:2011}. All details are provided in the appendix. NOW MOVE ALL OTHER TEXT TO THE APPENDIX?}


\subsection{Discretization}

\begin{wrapfigure}[4]{i}{0.21\linewidth}
\centering
    \begin{overpic}[scale=0.12]{triangle_fan3.pdf}
%\put(14,-5){$\mathbf{v}_j$}
%\put(-10,15){$\mathbf{v}_k$}
%\put(19,21){$\mathbf{v}_i$}
%\put(5,21){$e_{ik}$}
%\put(19,8){$e_{ij}$}

\put(37,-15){$\mathbf{v}_j$}
\put(-30,45){$\mathbf{v}_k$}
\put(56,59){$\mathbf{v}_i$}
\put(14,57){$e_{ik}$}
\put(51,21){$e_{ij}$}
\end{overpic}
\end{wrapfigure}
\sout{In the discrete setting, we approximate} \textcolor{red}{We discretize} shapes as manifold triangle meshes $(V,E,F)$, sampled at vertices $\mathbf{v}_i, i=\{1...|V|\}$, with the constraint that each pair of triangles $(\mathbf{t}_i,\mathbf{t}_j) \in F$ shares at most one edge $ e \in E$. Functions $f: \M \rightarrow \mathbb{R}$ are approximated at vertices with piecewise-linear basis elements; tangent vector fields $U:\M\to\mathcal{T}\M$ are constant within each triangle.

The gradient operator $\mathbf{G}\in\mathbb{R}^{3 |F| \times |V|}$ takes a function value per vertex $\mathbf{v}_i$ and returns a 3D vector per triangle $\mathbf{t}_{ijk} \in F$: %:V \rightarrow F$ is uniquely defined in term of the discretization of the metric $g$ induced by the parametrization from the unit triangle in the planar domain to its embedded representation in the higher dimensional Euclidean space.
 \sout{It is computed as:}
%
\begin{align*}
    \mathbf{G} f(\mathbf{t}_{ijk})\hspace{-0.05cm}=\hspace{-0.05cm} %\mathbf{g}_t^{-1}\nabla \tilde{f} =
    %\begin{pmatrix}e_{ij} & e_{ik}\end{pmatrix}
    \begin{pmatrix}\mathbf{v}_{j}^\top-\mathbf{v}_i^\top \\ \mathbf{v}_k^\top-\mathbf{v}_i^\top\end{pmatrix}^\top \hspace{-0.1cm}
    \begin{pmatrix} \|e_{ij}\|^2 & \hspace{-0.1cm}\langle e_{ij},e_{ik}\rangle  \\
     \langle e_{ij},e_{ik}\rangle & \hspace{-0.1cm} \|e_{ik}\|^2\end{pmatrix}\begin{pmatrix}  f(\mathbf{v}_j) - f(\mathbf{v}_i) \\ f(\mathbf{v}_k)- f(\mathbf{v}_i) \end{pmatrix}
\end{align*}
%
where the notation is as per the inset figure. % \MM{Why $Gf(v_i)$? $Gf(t_{ijk})$ or $Gf(v_i, v_j,v_k)$?}
%
 The divergence operator $\mathbf{D}\in\mathbb{R}^{|V| \times 3|F|}$ takes a 3D vector per triangle and returns a value per vertex. As the  adjoint of the gradient, it is discretized as : %
\begin{align}
\mathbf{D} = -\mathbf{A}^{-1}  \mathbf{G}^\top \mathbf{T}\,,
\end{align}
where $\mathbf{A}$ is a diagonal matrix of local area elements at each vertex (shaded area in the inset) and $\mathbf{T}$ is a diagonal matrix of triangle areas. %\MM{Is this the actual (numerical) adjoint? This  might be important for the numerics.}
%
These discretizations follow the standard formulations as described, e.g., in \cite{botsch2010polygon}.

To define these operators on point clouds, we base our approach on the construction of a graph $(\mathcal{V},\mathcal{E})$, built locally at each point in a $k$-neighborhood. The edges of the graph are weighted by a Gaussian kernel $w_{ij}=e^{-\frac{\|x_i-x_j\|_2^2}{\delta}}$\textcolor{red}{, for an appropriate $\delta$ depending on the point set density}. Functions $f: \mathcal{V} \to \mathbb{R}(\mathcal{E})$ are  defined on the nodes of the graph while vector fields $F: \mathcal{E} \to \mathbb{R}(\mathcal{V})$ are defined on the edges. The gradient and divergence operators are \sout{respectively} defined as: 
%
\begin{align}
    \mathbf{G}_{ij}&= w_{ij}( f_i - f_j) \ \ \ \forall (i,j) \in \mathcal{E}\\
    \mathbf{D}(F_i)&=\sum_{j \in (i,j) \in \mathcal{E}} \hspace{-0.2cm} w_{ij}(F_{ij}-F_{ji})
\end{align}


\sout{Finally,} In order to deal with low-quality meshes, we adopted the \sout{intrinsic triangulation} approach of \cite{sharp2019navigating}; a more detailed discussion with an experimental comparison is given in Appendix~\ref{sec:params}.

\subsection{Minimization of Eq.7}
%
The energy to minimize in line 3 of Alg.~\ref{alg:1} is convex, but non-differentiable. To efficiently solve it, %we leverage duality techniques from convex analysis. In particular
 we discretize the problem and use the primal-dual hybrid gradient algorithm~\cite{chambolle:2011}, which is well-suited for {\textcolor{red}{problems of this form.}} %
 \sout{
 %
 %
 %
  problems of the form:
%
\begin{align}\label{eq:pd}
    \min_{u} \mathcal{F}(K u) + \mathcal{G}(u)\,,
\end{align}
%
where $K$ is a linear operator \sout{(the discretization of the gradient in our case)}, and $\mathcal{F},\mathcal{G}$ are closed, convex, possibly not differentiable functions with easy-to-evaluate proximal operators. 
%
By Legendre-Fenchel duality, we can rewrite Eq.~\eqref{eq:pd} as a saddle point problem:
%
   \begin{align}
       \min_{u } \max_{q } \langle{K u,q} \rangle - \mathcal{F}^*(q) + \mathcal{G}(u)\,,
   \end{align}
%
where $\mathcal{F}^*(q) = \sup_v \left\{\langle q,  v \rangle - \mathcal{F}(v)\right\}$ is the convex conjugate of $\mathcal{F}$. % In our case, $\Omega=BV(\M)$ and $\Omega^*=BV(\mathcal{T}\M)$ \MM{Is this the dual of BV? Or the pre-dual? max or sup? safer to use the finite setting directly.}.
%
%In the discrete setting, we get: %\footnote{This formulation can also be directly obtained from the weak definition of the total variation in (\ref{dfn:dualTV})}
%$^{,}$\footnote{The regularization parameter now weights the fidelity term in an equivalent, but more adequate to mathematical computations, formulation}:
%
 We set $K = \mathbf{G}$ to be the discrete gradient, $\mathcal{F}^*$ to be the (triangle-wise) indicator function of the unit ${L}^2$ ball, and $\mathcal{G}(u) = \frac{1}{2\alpha}\|\mathbf{u}-\mathbf{u_0}\|_2^2$.}
%\begin{align} 
%    \min_{\mathbf{u} : V \to \mathbb{R}} \max_{\mathbf{q} : F \to \mathbb{R}^3} \mathbf{q}^\top \mathbf{G} \mathbf{u} - \chi_{B_2}(\mathbf{q}) + \frac{1}{2 \alpha}\|\mathbf{u}-\mathbf{u_0}\|_2^2\,,
%\end{align}
%
%with $\chi_{B_{2}}$ being the indicator function of the $\mathcal{L}^2$ unit ball $B_2$, such that $\chi_{B_{2}}(x)=0$ for $x \in B_{2}$, and $\chi_{B_{2}}(x)=\infty$ otherwise. %with $\chi_{B^*}$ being the indicator function of the  dual norm unit ball, with $B^*=B^2$ and $B^*=B^\infty$, when considering $BV_2(\M)$ and $BV_1(\M)$, respectively.
%
%\begin{align}
%    \chi_{B_{2}}(x)=\begin{cases} 0 & x  \in B_{2} \\
%    \infty & \text{otherwise}
%    \end{cases}
%\end{align}
The optimization procedure for an input signal $\mathbf{u}$ is summarized in Algorithm~\ref{PDHG}:
\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$\mathbf{u}$, $\mathbf{q}$, $\sigma,\tau>0$, $\theta \in [0, 1]$}
\Output{minimizer $\mathbf{u}^\ast$ of Eq.~\eqref{eq:1}}
\Begin{
	\While{not converged}{
		$\mathbf{u}_{k+1}=prox_{\mathcal{G},\tau}(\mathbf{u}_k - \tau \mathbf{D} \mathbf{q}_k)$\\
		$\bar{\mathbf{u}}_{k+1}=\mathbf{u}_{k+1}+\theta(\mathbf{u}_{k+1}-\mathbf{u}_{k});$\\
		$\mathbf{q}_{k+1}=prox_{\mathcal{F}^*}(\mathbf{q}_k + \sigma \mathbf{G} \bar{\mathbf{u}}_{k+1})$
		}
\Return $\mathbf{u}^\ast= \mathbf{u}_{k+1}$
\caption{\label{PDHG}Primal-Dual Hybrid Gradient (PDHG)}}
\end{algorithm}
%The algorithm alternates a proximal gradient descent step in the primal variable $\mathbf{u}$ (line 3), with a proximal ascent step in the dual $\mathbf{q}$ (line 5). Convergence is guaranteed, e.g. for $\theta=1$ and $\tau\sigma\leq \frac{1}{\|\mathbf{G}\|_{o}^2}$, where $\|\mathbf{G}\|_{o}$ denotes the operator norm of $\mathbf{G}$, see \cite{chambolle:2011} for details. 
%
the proximal operator $prox_{\mathcal{F}^*}$ \sout{of $\mathcal{F}^*$} is the projection of each component of its input onto the unit $L^2$ ball: 
%
\begin{align}
    prox_{\mathcal{F}^*}(\mathbf{q}_{j,:})= %\Pi_{B_2}(\mathbf{q})=
    \begin{cases}
\mathbf{q}_{j,:} & \|\mathbf{q}_{j,:}\| \leq 1 \\
\frac{\mathbf{q}_{j,:}}{\|\mathbf{q}_{j,:}\|} & \text{otherwise}\end{cases}\,,
\end{align}
%
where each $\mathbf{q}_{j,:}\in\mathbb{R}^3$ is a vector at triangle $j$.
%
%\MM{The above formula/notation is not quite correct. You have many points in space / triangle. At each triangle, $\mathbf{q}$ is a vector. Each of these vectors has to be projected onto the unit ball separately. Can you find some notation that is as consistent as possible to the code? E.g. $\mathbf{q}_{j,:}$?}
%
The proximal operator $prox_{\mathcal{G},\tau}$ \sout{with respect to the data fidelity term} has a closed-form solution given by:
%
\begin{align}
    prox_{\mathcal{G},\tau}(\mathbf{u})=\frac{\mathbf{u} + \frac{\tau}{\alpha}\mathbf{u}_0}{1+\frac{\tau}{\alpha}}\,.
\end{align}

We initialize the algorithm with $\mathbf{u}$ coming from the previous iteration in Algorithm~\ref{alg:1} and $\mathbf{q}=\mathbf{0}$, and stop the iterations when the absolute change in energy is below a small threshold. %\MM{Side remark: If I review publications that use this stopping criterion, I usually tell the authors that this is dangerous as not even a monotonic decay of the energy can be guaranteed for PDHG. PRimal and dual gaps are a better thing to track. For now, just leave it as it is.} 
We set $\theta=0.5$, which appeared optimal in \sout{terms of} our numerical experiments. 


==> Spectral TV (Copy)(3)/sections/intro.tex <==
\section{Introduction}
%
In the last decades, the computer graphics community has witnessed a thriving trend of successful research in computational spectral geometry. Spectral approaches have met with considerable traction due to their generality, compact representation, invariance to data transformations, and their natural interpretation relating to classical Fourier analysis. Despite these benefits, the vast majority of current spectral methods rely upon the construction of smooth basis functions (obtained, for instance, as the eigenfunctions of the Laplace operator), leading to significant detail loss whenever the signal to be represented is not smooth. When this signal represents geometric information (e.g., the $(x,y,z)$ coordinates of mesh vertices), this inevitably leads to a ``lossy'' geometric encoding, \sout{which is} typically manifest as over-smoothing, vertex collapse, or spurious oscillations (so called Gibbs phenomenon) not appearing in the original geometry.

Such artifacts derive from the \sout{very} motivations underlying the seminal work of Taubin~\shortcite{Taubin:1995} and follow-up \cite{Desbrun:1999}, which were posed as an extension of the diffusion techniques from image processing to mesh {\em smoothing} applications. Today, the key driver behind their continued adoption lies in the convenient representation, which enabled significant gaps in performance in many relevant problems (e.g., shape correspondence \cite{ovsjanikov2012functional,zoomout}, vector field processing \cite{brandt2017spectral} among many others), while still suffering from often undesirable effects.

%
\begin{figure}[t!]
\begin{center}
  \begin{overpic}
  [trim=0cm 0cm 0cm 0cm,clip,width=1.0\linewidth]{./images/teaser.png}
  \end{overpic}
  \caption{\label{fig:teaser}Our method allows us to \sout{isolate and} process the geometric details of a given shape into well separated spectral bands having different semantics. Each band corresponds to a different geometric feature, possibly not localized in space. In this example, the star decorations are removed from the knot via a simple low-pass filter in the TV spectrum. The method is rotation-invariant, as it does not depend on the orientation of the knot \sout{model} in 3D space.}
  \end{center}
\end{figure}
%

The present work finds its motivation in the fact that detail preservation is a strict necessity in a wide class of applications in graphics. We start from the observation that, similar to most natural images, shape geometry often has a sparse gradient. For a scalar function $f$, this quantity can be measured via the {\em total variation} functional:
%
\begin{align}
\label{eq:tv}
    TV(f) = \int || \nabla f(x) || dx\,,
\end{align}
%
which, for coordinate functions, captures the amount of sharp geometric variations in a given object.
%
Leveraging recent progress in image processing \cite{Gilboa:2013,Burger:2016}, we use the above functional to derive a {\em nonlinear} operator, the subdifferential $\partial TV$, which has numerous piecewise-constant functions as \emph{eigenfunctions}. 

Using the TV functional, we provide a spectral decomposition ({\em analysis}) algorithm for functions $f$ on a manifold which, similarly to Fourier decompositions, carries a canonical multiscale ordering, providing a sharp separation of the source signal into different bands; as a direct consequence to the sparsity of the gradient, frequency bands in the spectral domain assume a semantic connotation, and can be filtered and processed following classical signal processing paradigms (see Figure~\ref{fig:teaser} for an example). Importantly, since $TV(f)$ remains finite for a wide variety of discontinuous $f$ (with an appropriate adaptation of the definition~\eqref{eq:tv} to be discussed in Eq.~\eqref{dfn:dualTV}), discontinuities are preserved by the transform, \sout{which is} and is therefore well-suited for representing jumps and sharp high-frequency variations. The inverse transform ({\em synthesis}) is realized by a single linear step.

Our approach shares some common traits with Laplacian mesh processing, for which it provides a nonlinear alternative; in particular, we show that both settings can be derived as specific instances of a more general model.
%
We demonstrate the versatility of our framework by applying it with success to several applications in geometry processing and graphics, relating its multiple incarnations to existing ad-hoc approaches, and illustrating its performance across different settings and shape representations.
%


%The field of shape analysis has deeply benefited from the study of the spectrum of the Laplace Beltrami operator (LBO), whose eigedecomposition provides a way to generalize Fourier analysis to non Euclidean domains, allowing to express an arbitrary function defined on a surface as a superposition of smooth basis elements \cite{Aflalo:2014}. This framework supplies a way to perform countless tasks in computer graphics  \cite{Taubin:1995,Levy:2006,Reuter:2006}, which all benefits from the compact representation and the exposure of hidden information of the original datum in the spectral domain. 
%
%Despite its uncountable uses in shape processing and analysis, a well known drawback of this spectral representation is in the representation of discontinuous functions: this class of functions cannot be properly reconstructed as a finite linear combination of Fourier basis functions. In particular, since the standard practice in spectral geometry is to work with a truncated basis of LBO eigenfunctions due to computational efficiency reasons, discontinuities are approximated with smooth transitions and are not preserved in the reconstructed signal (see Figure~\ref{fig:gibbs}).
%
%Nonetheless this class of functions is of fundamental importance in the field of computer graphics: it includes the class of step functions, which have key applications in segmentation or partial shape matching. Moreover when choosing a function which provides a description of the surface itself, discontinuities in the function correspond to the details of the shape. 
%
%In this work we propose an alternative nonlinear operator which is derived from the total variation functional whose spectrum provides a sparse multiscale representation for functions defined on surfaces, which is optimal for representing discontinuities.



\subsection{Contribution}
%
With this paper we introduce a new framework for geometry processing that weaves discontinuity-preserving regularization into the fabric of a spectral approach.
%
Our key contributions are:
%
\begin{itemize}
    \item We introduce a general {\em spectral} framework to analyze and process non-smooth signals defined on surfaces, as well as the surfaces themselves, which fully preserves geometric detail; %for the first time, we bring this framework from the Euclidean case to curved surfaces;
    \item We adopt a fast, unconditionally stable algorithm to solve the resulting nonlinear problem on non-Euclidean domains, with limited dependence on a few parameters;
    \item We analyze the evolution of surfaces along the flow induced by the operator, and relate it to existing geometric flows\sout{, and further inspect the commonalities with the Laplace-Beltrami operator}\sout{verifying that they both are particular cases of a more general operator};
    \item We explore a wide range of possible applications in shape analysis and modelling, where we compare to state-of-the-art methods in the respective domains, demonstrating production quality results in many cases.
\end{itemize}

==> Spectral TV (Copy)(3)/sections/method.tex <==
\section{Spectral TV decomposition}
%
%Classically, signal processing involves the definition of an invertible map to transform a given signal into a ``frequency'' domain (analysis), and back to the primal space (synthesis). The forward transform decomposes the signal into several subspaces, each associated with a different scale, exposing information that was hidden in the original representation. Crucially, manipulation of these components, as well as the signal reconstruction, can be done easily.
%
%given a signal represented in a certain space, one aims to define an invertible map to transform it in a different domain, which result as the decomposition of the former into subspaces associated with different frequencies or scales. This spectral representation allows to expose information proper of the signal, which is typically hidden in the original representation. One can then operate on the spectral domain by acting on the single frequencies and then reconstruct the signal in the original domain, leveraging on the invertibility of the transform.
%
%We highlight the following facts, which characterize the transform  considered in this work:

In this work we introduce a new invertible transform for signals defined on surfaces, with the following key properties:
%
\begin{itemize}
    \item The forward transform is non-linear;
    \item The inverse transform is linear;
    \item Any signal $f\in BV(\M)$ on the surface can be decomposed and reconstructed up to a desired accuracy;
    \item Discontinuities in $f$ are preserved by the transform.
\end{itemize}
%\MM{please see if the following statement is ok with you:}
The following considerations closely follow the ideas of \cite{Gilboa:2013, GuySpectralSiam14} in the Euclidean setting, but extend them to functions on manifolds to enable discontinuity-preserving geometry processing.
%\MM{I'd say we can delete these two sentences:}\textcolor{green}{(Marco) Good to me}The transform is based upon the definition of a diffusion process that is designed to preserve discontinuities in the signal. The diffusion operator is nonlinear, and admits a notion of generalized eigendecomposition that we directly exploit in the applications.


\subsection{TV flow}
%
Consider the following energy for surface signals $u,u_0\in BV(\M)$:
%
\begin{equation} \label{eq:energy}
E(u) = \frac{1}{2}\int_\mathcal{M}(u(x)-u_0(x))^2 dx+ t TV(u)\,, \quad t>0
\end{equation}
%
with the associated variational problem: 
%
\begin{equation}\label{eq:1}
\min_{u\in BV(\M)} E(u)\,. % = \min_{{u\in  BV(\M)}}{||u-u_0||_2^2 + t TV(u)}
\end{equation}

The above seeks to minimize a functional over two terms: a \textit{fidelity term}, which quantifies the distance from an initial function $u_0$, and a \textit{regularization term} which measures the total variation of the sought minimizer. The regularization parameter $t$ balances between the two terms. 
%
In image processing, where $\mathcal{M} = S \subset \mathbb{R}^2$, Eq.~\eqref{eq:1} is known as the ROF model for image denoising \cite{Rudin:1992}, and dissipates noise in flat regions of an image $u_0$ while preserving object contours.

Iteratively applying Eq.~\eqref{eq:1} to the output of a previous solution with small increases of $t$ can be seen as a discretization of a time continuous \textit{total variation flow}: %\MM{I recommend to omit the appendix apx:euler}
%Solving the Euler-Lagrange equations of the energy $E$ with Neumann boundary conditions yields the following PDE (Appendix~\ref{apx:euler}):
%
\begin{align}\label{eq:pde}
    \begin{cases}
    \frac{\partial u}{\partial t}= ~\mathrm{div} \left(\frac{\nabla u}{\|\nabla u\|}\right) &  \text{in  } \M,\\
    \langle \nabla u , \vec{n} \rangle=0 & \text{on  }  \partial \M , \\ 
    u(0,x) = u_0,
    \end{cases}
 \end{align}
%
where $\vec{n}$ is the unit vector normal to the boundary $\partial\M$. Equations~\eqref{eq:pde} describe a physical process of isotropic diffusion within the level sets of the initial function $u_0$, without any diffusion across them (see Figure~\ref{fig:TVflowsphere}). In $\mathbb{R}^n$, it is guaranteed that the flow converges in finite time to a constant solution under mild assumptions \cite[Cor.~1]{andreu:2002}; no proofs exist for manifolds, but in our experiments we always observed convergence.

To give sense to Eq.~\eqref{eq:pde} for nondifferentiable $u$ and points at which $\nabla u(x)=0$, one needs to turn to the \textit{subdifferential}, which for a convex functional $J$ (TV in our case) over a function space $\mathcal{X}$ is formally defined as the set:
%
\begin{align*}
    {\partial J}(u) =
    \left\{ p \in \mathcal{X}^* ~|~  \ J(v) - J(u) \geq  \langle p,v-u\rangle, \ \forall v \in \mathcal{X} \right\}\,,
\end{align*}  
%
with $\mathcal{X}^*$ being the dual space of $\mathcal{X}$. For smooth $u$ with non-zero gradient one obtains:
%This model is fully governed by the nonlinear operator:
%
\begin{align}\label{eq:dtv}
    \partial TV (u) = \left\{ -\mathrm{div} \left(\frac{\nabla u}{\|\nabla u\|}\right)\right\}\,.
\end{align}
%
%i.e., the subdifferential of $TV$ at $u$. 
%\MM{for smooth $u$ with non-zero gradient.
We refer the reader to \cite{bellettini:2002} for more details on the TV flow in a Euclidean setting.





%We recall that the subdifferential of a convex functional $J$ over the function space $\mathcal{X}$ is formally defined as the set:
%
%\begin{align}
%    {\partial J}(u) =
%    \left\{ p \in \mathcal{X}^* ~|~  \ J(v) - J(u) \geq  \langle p,v-u\rangle, \ \forall v \in \mathcal{X} \right\}\,.
%\end{align}
%
%In our case $J=TV$, and $\partial TV$ corresponds to the element in $\partial J$ with minimum norm.

%Since the TV functional is not differentiable everywhere, we recall that the subdifferential is formally defined as the set:
%
%\begin{align}
%    \widetilde{\partial TV}(u) &= \\
%    &\left\{ p \in \mathcal{L}^2(\M) ~|~  \ TV(v) - TV(u) \geq  \langle p,v-u\rangle, \ \forall v \in \mathcal{L}^2(\mathcal{M}) \right\}\nonumber
%\end{align}
%
%Eq.~\eqref{eq:dtv} corresponds to the function in $\widetilde{\partial TV}(u)$ with minimum norm.


\begin{figure}[t]
  \centering
\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=1.0\linewidth]{images/spheres-disk.png}
\put(4,-3){\footnotesize $t=0$}
\put(23,-3){\footnotesize $t=0.05$}
\put(44.5,-3){\footnotesize $t=0.1$}
\put(65,-3){\footnotesize $t=0.2$}
\put(85.5,-3){\footnotesize $t=0.3$}
%
\put(99.7,9.5){\tiny $0$}
\put(99.7,13.5){\tiny $1$}
\end{overpic}
  \caption{\label{fig:TVflowsphere}Evolution of a disk-shaped function along the TV flow on a spherical surface. Since the diffusion only acts {\em inside} the level sets, the disk preserves its shape and loses contrast linearly until it vanishes.% See Fig.~\ref{fig:sol1dflow} (first column) for an analogous example in 1D.
  }
\end{figure}

\subsection{Nonlinear eigenvalue problem}
%

A generalized eigenfunction of the operator $\partial J$ is a function $u$ with $\|u\|=1$ satisfying the following relation for some number $\lambda\in\mathbb{R}$ (its corresponding generalized eigenvalue):
%
\begin{align}\label{eq:eigentv}
    \partial J(u) \ni \lambda u\,,
\end{align} 
%
where $J=TV$ in our case. %\MM{I think we should require $u$ to be normalized, $\|u\|_2 = 1$.}
%Where the dependence on  the eigenfunction $u$ is non linear and equality is replaced by an inclusion in the set $\partial TV(u)$. %, which is the subdifferential of $TV$ at $u$:
%
%equivalent characterization of \partial TV which follows from the one homogeneous property of TV
%\begin{align}
%    \partial TV(u)=\left\{ p \in \mathcal{L}^2(\M) | \langle{p,v} \rangle_\M \leq TV(v), \ \langle{p,u} \rangle_\M  = TV(u), \ \forall v \in \mathcal{L}^2(\mathcal{M}) \right\} 
%\end{align}
This relation generalizes the classical characterization of eigenpairs of a linear operator: %For one-homogeneous functionals $J$, it can be easily proven that the subdifferential satisfies $J(u) = \langle p,u\rangle$ for all $p \in \partial J(u)$ (see e.g. \cite[Lemma 3]{Burger:2016}). It is interesting to see that Definition \eqref{eq:eigentv} is a strict generalization of the classical notion of eigenvectors, e.g. for the Dirichlet functional:
%We can therefore see the classical Laplacian eigendecomposition as a special instance of Eq.~\eqref{eq:eigentv}: \MM{Why do we need the statement about one-homogeneous functions? The Dirichlet energy in the following remark is not one-homogeneous such that I find the conjunction "Therefore" in the previous sentence irritating.}

\begin{remark}
For the Dirichlet functional $D(u) = \frac{1}{2}\int_\M \| \nabla u \|^2$, one obtains $\partial D(u) = \{-\Delta u\}$, such that the analogy to Eq.~\eqref{eq:pde}  becomes the standard diffusion equation, and Eq.~\eqref{eq:eigentv} reduces to the standard eigenvalue problem $\Delta u = \lambda u$ (up to a sign). %The inclusion relation is replaced by an equality, since $D(u)$ is differentiable everywhere and thus $\partial D(u)$ is single-valued.
\end{remark}

%The generalized TV eigenvalues form a continuous spectrum~\cite{}. %, thus the associated eigenfunctions are uncountably many.

%We now study the behavior of generalized eigenfunctions under the TV flow.

\subsection{The TV flow on eigenfunctions}
\label{section:4:3}
%
Let us recall the ideas from \cite{Gilboa:2013, Gilboa:2015} to motivate a spectral decomposition using the TV flow. For eigenfunctions $u_0:\M\to\mathbb{R}$ with eigenvalue $\lambda$, we get a simple analytic solution to the flow of Eq.~\eqref{eq:pde}:
%
\begin{align*} %\label{tv:soltv1}
    u(t,x)=\begin{cases}
    (1 - t \lambda) \, u_0(x) & \text{for   } t \leq \frac{1}{\lambda} \\
    0  & \text{otherwise}
    \end{cases}
\end{align*}
%
At each point, the eigenfunction decreases linearly at increasing $t$, until it goes to zero. In other words, TV eigenfunctions preserve their shape (up to rescaling) under the action of the flow; Figure~\ref{fig:TVflowsphere} illustrates one such eigenfunction. 

The first derivative of $u(t,x)$ w.r.t. time is \sout{the} piecewise-constant\sout{ function}:
%
\begin{align*} %\label{tv:soltv2}
    \partial_t u(t,x)=\begin{cases}
     - \lambda u_0(x) & \text{for   } t \leq \frac{1}{\lambda} \\
    0  & \text{otherwise}
    \end{cases}
\end{align*}
%
Considering also the second derivative (in a distributional sense), we get a delta function placed exactly at the point in time where the solution $ u(t,x)$ vanishes (see Figure~\ref{fig:sol1dflow}):
%
\begin{align*} %\label{tv:soltv3}
    \partial_{tt} u(t,x)=\begin{cases}
    + \infty & \text{for   } t = \frac{1}{\lambda} \\
    0  & \text{otherwise}
    \end{cases}
\end{align*}
%
\begin{figure}
\centering%
\includegraphics[width=\linewidth]{images/plot_eigen.png}
%\input{images/plot.tex}%
\caption{\label{fig:sol1dflow}Analytic solution (left) to the 1D flow for a TV eigenfunction $u_0$ with eigenvalue $\lambda=\frac{1}{3}$, first and second derivatives (resp. middle and right).}%
\end{figure}
%
\sout{We see that} The behavior of the second derivative $\partial_{tt} u(t)$ for an eigenfunction $u_0$ resembles \sout{bears a strict resemblance with} the notion of spectrum in \sout{classical} Fourier analysis, since sinusoidal functions (eigenfunctions of the Laplace operator) correspond to \sout{are represented as} deltas \sout{functions} in the frequency domain. 
%
This motivates the definition:
%
\begin{defn}
\label{def:spectralRepresentation}
We refer to the distribution over time $\phi_t= \partial_{tt} u(t)$ as the {\em spectral representation} of $u_0$, and to each individual distribution at the time scale $t$ as a {\em spectral component}. 
\end{defn}
%
As we have seen, for a TV eigenfunction with eigenvalue $\lambda$, the spectral representation has a single component: \sout{which is} a delta at $t=\frac{1}{\lambda}$. %For a generic function, its spectral representation is supported over an interval in $t$.
%
However, not every spectral component $\phi_t$ is guaranteed to identify a TV eigenfunction. 
Further, at any given time scale $t$, the spectral component $\phi_t:\M\to\mathbb{R}$ still has a spatial extent over $\M$. 
%is a function \MM{(not really)} defined over $\M$. 
To show the entire spectral activity across different time scales, we can integrate each $\phi_t$ and simply plot the function: %\MM{strictly speaking, this is not justified. To show the entire spectral activity across different time scales, we sum the absolute values of the discrete representation of $\phi_t$ over the manifold, formally corresponding to a continuous formulation}
%
\begin{align}
\label{eq:spectrum}
s(t)=\int_\M |\phi_t(x)| dx\,.
\end{align}
%
%\MM{while being aware that this is challenging }
Looking at the behavior of the function $s(t)$ can be rather useful in practice, since it helps in defining the filtering operations required by the applications; examples of $s(t)$ are shown in Figure~\ref{fig:teaser}.

%In other words, computing the {\em forward} TV transform of a signal $u_0$ on a surface $\M$ boils down to computing its spectral components.
%
The spectral representation can be translated back to the primal domain by the linear operation of integrating over time (i.e., across all spectral components $\phi_t$) and adding the mean of $u_0$: %\MM{One can only reconstruct $u_0$ up to a constant (assuming that also on a manifold $TV(u)=0$ implies that $u$ is constant).}
%
\begin{align}\label{eq:inv}
 u_0= \int_0^\infty t \phi_t dt \, + \text{mean}(u_0)\,.
\end{align}
%
We refer \sout{the reader} to \cite{Gilboa:2013, GuySpectralSiam14} for more details (with the slight difference that we decided to define the spectral decomposition without the factor $t$ and include it in the reconstruction instead). %Also, we note that quantities like \eqref{eq:spectrum} are problematic from a functional analytical perspective. Yet, similar to \cite{GuySpectralSiam14} it nicely illustrates the behavior in the discretized case, i.e., in the numerical experiments. For a more precise mathematical perspective we refer to \cite[Sec. 3.5]{Burger:2016}. 

%The integral converges, since $\phi_t$ originated from a finite-time flow. % holds because eigenfunctions change only finitely many times during the flow (see \cite{Burger:2016}).


\subsection{The spectral representation induced by the TV flow}\label{sec:dict}
In light of the previous discussion that TV eigenfunctions are the fundamental atoms of the spectral representation of Def. \ref{def:spectralRepresentation} (in the sense that they yield peaks in the spectral domain), one might expect to represent arbitrary signals as linear combinations of such atoms. 
%
Although there seems to be a vast number of TV eigenfunctions to allow such a representation\footnote{See e.g. \cite{Steidl:2004} for a proof that the Haar basis is a proper subset of the TV eigenfunctions on the real line, or \cite{Alter05} for a characterization of sets whose characteristic function is a TV eigenfunction.}, computing a \sout{reasonable (i.e.,} \textit{sparse} \sout{)} representation turns out to be difficult since, e.g., a Rayleigh principle to compute orthogonal eigenfunctions does not hold \cite{Benning:2013}.

Interestingly, Def.~\ref{def:spectralRepresentation} allows to show that the gradient flow with respect to a regularization with suitable properties does yield such a decomposition with the $\phi_t$ representing differences of eigenfunctions, see \cite{Burger:2016}. 
%, Bungert19}.
 While the TV in Euclidean spaces of dimension larger than $1$ does not satisfy the required properties, the spectral representation $\phi_t$ has been shown to still yield a meaningful, edge-preserving, data-dependent multi-scale representation in the field of image processing \cite{GuySpectralSiam14, Gilboa:2015}, which is why we utilize it on manifolds in a similar fashion.


%Since TV eigenfunctions preserve their shape under the TV flow, one may think that this is true for a very large class of functions. Indeed, the three piecewise-constant functions (one on each flag) shown in the inset are TV eigenfunctions, each with a different eigenvalue, and where only the leftmost has connected support. %\MM{Really? The middle one has two very close objects that will be connected under the TV flow. The right one has points of infinite curvature, which should never result in a TV eigenfunction...}

%TV eigenfunctions form an overcomplete dictionary\footnote{To be precise: Overcompleteness was proven on the real line \cite{Steidl:2004} by showing that the Haar basis is a proper subset of the TV eigenfunctions. We conjecture that the same holds on manifolds w.r.t. Haar-like bases such as \cite{girardi1997new}, but a rigorous proof is still an open problem and is left for future work.} for the function space $BV(\M)$: %
%\begin{align}
%    \mathcal{D} = \left\{ u  \in BV(\M) \   | \ \ \lambda u =- \mathrm{div} \left(\frac{\nabla u}{\|\nabla u\|} \right)\right\}\,.
%\end{align}
%
%We conjecture that -- at least in the discrete case -- any arbitrary function can be represented as a linear combination of eigenfunctions, but the choice of the dictionary elements is not unique. It is therefore an ill-posed problem with more solutions than unknowns.
%
%Next we show a strategy to drive this choice.

%\begin{remark}
%By invoking the notion of a dictionary, we follow the same principle behind compressed sensing approaches \cite{candes2006stable}, which enable nearly exact representation of sparse signals with few elements of a dictionary. Here we adopt the same assumptions, namely that our signals of interest are sparse in the {\em gradient} domain.
%\end{remark}
%\MM{Again, good link, but finite vs. infinite-dimensional setting is problematic. Maybe there is a way to make the overall paper a little more precise (or purposefully vague) with respect to the considered setting. }
% straightforward to obtain since the Haar basis (together with the concept of dilation and translation implied) is not possible to define in a classical manner on curved domains.


\subsection{Computing the TV spectral decomposition}
\label{section:4:5}
%The procedure described in the section 3.4 can be generalized to transform arbitrary signals into the TV spectral domain.
%Due to the overcompleteness of the dictionary of TV eigenfunctions we can represent a given signal with less elements than those required with the underlying basis alone, obtaining a sparse representation of it. On the contrary, since we have different choices between the elements in the dictionary with which we can represent a given signal, 
%
To compute the spectral representation $\phi_t$ of a given function $f$, we use an implicit Euler discretization of the TV flow: We compute a new iterate by solving \sout{the ROF model of} Eq.~\eqref{eq:1} using the previous iterate in the data fidelity term starting from $u_0 \equiv f$. % and compute the next iterate by applying  in the fidelity term of Eq.~\eqref{eq:1}, and study the evolution of the signal under the action of the TV flow.
%
%To solve the overdeterminate problem we introduce the idea of \textit{eigedecomposition guided by data}, which exploits the fidelity term in problem \eqref{eq:1}.
%This way, the choice of the elements of the dictionary is constrained by the data, and a unique representation can be obtained for the input signal.
%
The procedure is summarized in Algorithm~\ref{alg:1}.

\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{signal $u_0$, step length $\alpha$, no. of time steps $N$}
\Output{spectral representation $\phi_t$}
\Begin{
	\For{$t=0:N$}{
		$u(t) \xleftarrow{Alg. \ref{PDHG}} \min_u TV(u) + \frac{1}{2 \alpha} || u- u_0||_2^2 $\\
		output $\phi_t \xleftarrow{} \partial_{tt} u(t)$ \\
		increase $\alpha$ \\
		update $u_0$ ${\xleftarrow{} u(t)}$
			}
\caption{\label{alg:1}Spectral TV decomposition}}
\end{algorithm}
%
The algorithm simply evolves the input signal by $N$ discrete steps along the TV flow; each iteration moves a step forward, with diffusion time equal to $\alpha$. As changes happen quickly for small $t$ and tend to become slower for larger $t$ we iteratively increase the step size $\alpha$ of the evolution. Subsequently, the spectral representation $\phi_t$ is constructed incrementally using finite differences, such that the integral of Eq.~\eqref{eq:inv} becomes a simple weighted sum over the $\phi_t$. We give selection strategies for $\alpha$ and $N$ in Appendix~\ref{sec:params}.


\begin{figure}
    \centering
     \includegraphics[width=0.9\linewidth,trim={0 0 0 0},clip]{images/duck.png}
      \caption{\label{fig:duck}Spectral TV transform \sout{of a color signal} on a rubber ducky. The original signal (top left) is composed of three indicator functions of different regions, \sout{which are} represented in the TV spectral domain as three separated peaks (top right). Each plot visualizes the spectral activity \sout{$s(t)$} of the corresponding surface signal\sout{, defined as  $s(t)=\int_\M |\phi_t(x)| dx$}. By filtering the peaks in the spectral domain we can single out each component at a different scale, obtaining one region at a time (bottom row).}
      
\end{figure}
%\vspace{-1cm}
\begin{figure}[b!]
    \centering
\begin{overpic}[width=\linewidth]{./images/cow.png}
\put(10.5,-1){\footnotesize source}
\put(48,-1){\footnotesize filtered A}
\put(80,-1){\footnotesize filtered B}
\end{overpic}
\caption{\label{fig:cow}The source surface signal (left) is transformed into a spectral TV representation, and processed with two band-pass filters to obtain a cow without eyes and nostrils (A) and without spots (B).}
\end{figure}

\begin{remark}
This yields a {\em multiscale} representation for the input, since each diffusion time $t$ captures a feature at a different scale -- namely, the feature that vanishes at $t$. Here, time scales play the same role as a wavelength in classical Fourier analysis. %\MM{For small times $t$ only the most oscillating patterns (=highest frequency) vanishes. Thus the interpretation of $t$ should be the wavelength rather than the frequency, shouldn't it? } % The activity at each frequency is measured by the $L^1$ norm of the spectral components $\phi_t$.
\end{remark}

See Figures~\ref{fig:duck} and \ref{fig:cow} for examples of multiscale TV decomposition of color signals on two different surfaces.



%In terms of TV eigenfunctions, the decomposition $\phi_t$ of $u_0$ can be expressed as:
%
%\begin{align}
%    \phi_t=\partial_{tt}u(t) &=\lim_{\epsilon \to 0} \frac{\partial_t u(t+\epsilon) -\partial_t u(t)}{\epsilon} \\
%    &= \lim_{\epsilon \to 0} \frac{\lambda_t u(t+\epsilon) -\lambda_{t+\epsilon} u(t)}{\epsilon}\,,
%\end{align} 
%
%where $u(t), u(t+\epsilon) \in \mathcal{D}$, and $ \lambda_t, \lambda_{t+\epsilon}$ are their corresponding eigenvalues. Therefore, the computed spectral components of the signal $u_0$ correspond to the change of the eigenfunctions along the flow.  \MM{This is confusing to me, why should $u(t)$ be an eigenfunction? In previous works we showed that under certain conditions the $\phi_t$ are differences of eigenfunctions, but this is unclear here. Unless we have a solid mathematical understanding, I think it is safer to refer to previous works instead of using equations (18) and (19).}
    
%This allows us to obtain a multiscale representation of the signal which has the key feature of preserving the discontinuities in it.
%The regularization parameter $\alpha$ plays a key role in the process as it is directly proportional to the time of diffusion, so increasing its value corresponds to move forward in the flow.

%
%\begin{remark}
\vspace{1ex}\noindent\textbf{Algorithmic considerations}. Algorithm~\ref{alg:1} is unconditionally stable, and line 3 corresponds to taking an implicit Euler step along the discretized TV flow. This property allows us to use arbitrary values for the step size $\alpha$ (therefore, the resolution of the decomposition) without compromising convergence. %\textcolor{red}{; for any $\alpha>0$ the discrete TV flow is guaranteed to converge to a constant solution in finite time}. 
%
 In practice, in our experiments we use a variant of Algorithm~\ref{alg:1} and study the evolution of the flow backwards in time by following a nonlinear inverse scale approach,
 %\cite{burger:2006},
 that starts from a constant solution and converges to the initial function $u_0$. The spectral decompositions of both approaches are very similar in practice and have been proven to be identical under certain assumptions, see \cite{Burger:2016}. The inverse scale variant comes with additional numerical robustness. \sout{, as remarked in the Appendix.} %This additionally brings extra robustness to the variability in scale of the input signal. 
The complete algorithm, along with a detailed discussion on the two flows and on the role of $\alpha$ are given in Appendices~\ref{apx:inverse} and~\ref{apx:inversecomp}.%\MM{So all numerical experiments are based on the inverse scale space flow? If so, shouldn't we base the entire paper on it? It seems unfair to discuss properties of the TV flow but do somethings entirely different in the numerics... Or vice-versa: Why not use the TV flow in the numerics?}
%\end{remark}
%


%\begin{figure*}[t]
%  \centering
%  \includegraphics[width=\textwidth,trim={0 10cm 0 0},clip]{spheres2.png}
%  \begin{Overpic}[grid]{
%  \resizebox{\textwidth}{!}{\input{images/plottt.tex}}}
%  \end{Overpic}
%  \caption{\label{fig:spectralTV}TV transform of an indicator function on a sphere: the original signal is composed of three indicator functions of regions of different areas, which are represented in the TV spectral domain as three separated peaks. By filtering the peaks in the spectral domain we can reconstruct the signal and single out the components at a given scale, obtaining only one region at a time.}
%\end{figure*}

\subsection{Properties of TV eigenfunctions}\label{sec:props}
%
We conclude by giving a more complete characterization of the TV eigenfunctions on surfaces. %, and clarify some aspects that are taken for granted, e.g., with Laplace-Beltrami eigenfunctions.
%
%\vspace{1ex}\noindent\textbf{Geodesic convexity.}
%
On the image domain, Bellettini et al.~\shortcite{bellettini:2002} proved that any indicator function $\chi_S :\mathbb{R}^2 \to \{0,1\}$ of a {\em convex} closed subset $S \subset \mathbb{R}^2$ is a TV eigenfunction with eigenvalue $\lambda=\frac{Per(S)}{|S|}$ if it satisfies the \sout{following} isoperimetric \textcolor{red}{inequality}\sout{requirement}:
%
\begin{align*}\label{eq:ratio}
     \max_{q  \in \partial S} {k}(q) \leq \frac{Per(S)}{|S|}\,,
\end{align*}
%
\sout{This inequality states} \textcolor{red}{requiring} \sout{that} the maximal curvature $k$ of \sout{the boundary of $S$} $\partial S$ \sout{must} \textcolor{red}{to} be less than or equal to the perimeter-area ratio of $S$, intuitively \sout{, this excludes} \textcolor{red}{excluding} oblong \sout{or excessively thin} regions.

Such results have later been generalized to $\mathbb{R}^n$ as well as to unions of such convex sets, where the convex sets need to be sufficiently far apart for the TV spectral decomposition to yield a single $\delta$-peak for each of the subsets, see \cite{Alter05}.
%
%If the indicator function $\chi_S$ identifies {\em disconnected} subsets of the domain, the convexity and isoperimetric requirements are applied to each individual component. \MM{Where does this result come from? I am pretty sure this is not correct. The two disconnected sets also need to be far enough apart from one another!}
%
\setlength{\columnsep}{7pt}
\setlength{\intextsep}{1pt}
\begin{wrapfigure}[3]{r}{0.42\linewidth}
\begin{center}
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=1.0\linewidth]{./images/convex.png}
\end{overpic}
\end{center}
\end{wrapfigure}
%
We conjecture (and consistently confirmed in all our experiments) that this result can be generalized to surfaces by replacing \sout{the convexity requirement} \textcolor{red}{convex subsets} with \sout{the notion of} {\em geodesically convex} subsets of surface $\M$, making the \sout{three} examples in the inset figure eigenfunctions of the \sout{total variation} \textcolor{red}{TV} on a manifold.
%
A patch $C \subset \M$ is geodesically convex if, given any two points $p,q \in C$, there exists a unique minimum-length geodesic \sout{$\gamma:[p,q] \to \mathcal{M}$} %s.t. $\min \int_p^q g(\dot{\gamma(t)},\dot{\gamma(t)}) dt$,
 connecting them which lies entirely in $C$. 
 %
 \sout{This means that} \textcolor{red}{Therefore} in certain practical cases (e.g., the cow's nostrils in Figure~\ref{fig:cow}) one actually gets TV eigenfunctions in the spectral decomposition\sout{ of the given signal}.
 
% \setlength{\columnsep}{7pt}
%\setlength{\intextsep}{1pt}
%\begin{wrapfigure}[5]{r}{0.45\linewidth}
%\vspace{-0.12cm}
%\begin{center}
%\begin{overpic}
%[trim=0cm 0cm 0cm %0cm,clip,width=1.0\linewidth]{./images/shirt.png}
%\end{overpic}
%\end{center}
%\end{wrapfigure}
%

\begin{figure}
    \centering
\begin{overpic}[width=0.9\linewidth]{./images/figure_shirt.png}
\put(10.5,-1){\footnotesize Input}
\end{overpic}
\caption{\label{fig:shirt}
A U-shaped function (left) is decomposed as a linear combination of TV eigenfunctions corresponding to two geodesically convex sets, \sout{which are} manifested as two peaks in the TV spectrum. Functions are color-coded, growing from blue (negative values) to red (positive values).}
\end{figure}


\begin{figure}[hb!]
    \centering
\begin{overpic}[width=0.87\linewidth]{./images/bimbe.png}
\put(10,13){\footnotesize Input}
\put(39,39){\footnotesize $\phi_{27}$}
\put(61.5, 33){\footnotesize $\phi_{38}$}
\put(82,25){\footnotesize $\phi_{46}$}
\put(88,4){\footnotesize $\phi_{60}$}
\end{overpic}
\caption{\label{fig:spectral_bimbe}Spectral TV decomposition of the mean curvature function on the bimba (left). The \sout{resulting} spectral components $\phi_t$ are visualized at increasing index. The curve plot shows the spectral activity function $s(t)$ of Eq.~\eqref{eq:spectrum}. Low frequency components localize on semantically relevant regions (the chignon), while higher frequencies localize along feature lines (the hair strands).}
\end{figure}

 In Figure~\ref{fig:shirt} we show an example of indicator function of a {\em non}-geodesically convex set (U-shaped, left) that can be represented by a linear combination of indicator functions of geodesically convex sets (right). In Figure~\ref{fig:spectral_bimbe} we show the spectral components of a more complex signal (the mean curvature); in this case, the components are not geodesically convex but we still get a meaningful decomposition that can be used for mesh processing.
 
 
 %Note also that all three examples in the inset figure of Section~\ref{sec:dict} satisfy geodesic convexity for each component.\MM{Fix this - disconnected sets} %While currently we have no proof that geodesic convexity is sufficient to characterize TV eigenfunctions on surfaces, in all our experiments we observed that this property always holds.
 
 \begin{comment}
\vspace{1ex}\noindent\textbf{No Rayleigh principle.}
%
Recall by Theorem~\ref{th:perimeter} that $Per(S)=TV(S)$, and in addition $|S|=\|\chi_S\|$. The ratio appearing in Eq.~\eqref{eq:ratio} thus corresponds to a generalized Rayleigh quotient, whose minimization leads to the first eigenvalue of the total variation $\lambda_1=\min_u \frac{TV(u)}{ \|u\| }$. In the linear case (e.g. when replacing $TV$ by the Laplace-Beltrami operator $\Delta$), one can exploit this principle to compute subsequent eigenvalues by constraining the optimization to the orthogonal subspace spanned by the previously computed eigenfunctions. However, in the nonlinear case orthogonality holds only with respect to the first \textcolor{red}{(constant)} eigenfunction \sout{(which is constant)}, and is not guaranteed for subsequent ones \cite[Sec. 3.3]{Benning:2013}.
%
Since the Rayleigh principle fails, a generalized Courant-Fischer theorem for the TV functional cannot be established, and we cannot decompose our nonlinear operator into an orthonormal basis. This further motivates the need for the data-driven approach described in Section~\ref{section:4:5}. \MM{The word orthonormal basis might need clarification - the Banach space BV does not have an inner product. But is is reasonable to embed this into $L_2$.}
\end{comment}

==> Spectral TV (Copy)(3)/sections/preliminaries.tex <==
\section{Mathematical Preliminaries}

%say somewhere that our prior is that there is a sparse gradient; this prior makes the ill-posed problem tractable

\subsection{Surfaces}
%
We model shapes as compact and connected Riemannian manifolds $\M$ embedded in $\mathbb{R}^3$, possibly with boundary $\partial\M$, and with tangent bundle $\mathcal{T}\M =\bigcup_{p \in \M} \mathcal{T}_{p} \M$. The manifold is equipped with a metric, i.e., an inner product defined locally at each point, $\langle \cdot,\cdot\rangle_p: \mathcal{T}_{p}\M \times \mathcal{T}_{p}\M \rightarrow \mathbb{R}$, making it possible to compute lengths \sout{, areas,} and integrals on $\M$. 
%\begin{align}
%&\int_\M f(x) dx= \int\int_\Omega f(u,v)\sqrt{\det{g}} du dv \\
%&\langle{f,g}\rangle_{M}=\int_\M f g  \ dx \\
%& \langle{U,V}\rangle_{\mathcal{T}\M}=\int_\M g(U, V)  \ dx
%\end{align}
%Where $\Omega \subset \mathbb{R}^2$ is the parametric domain.
 The intrinsic gradient $\nabla_{\M}$, defined in terms of the metric, generalizes the \sout{classical} notion of gradient to manifolds; %and is defined locally in terms of the metric as:
%\begin{align}
%&\nabla_{\M}f (p)= g_p^{-1} \nabla  f(p) = g^{-1} \left(\frac{\partial}{\partial u} f(u,v), \frac{\partial}{\partial v} f(u,v)\right) \,.
%\end{align}
%
 similarly, the intrinsic divergence $\mathrm{div}_\M$ \sout{generalizes the notion of divergence and} can be defined as the negative adjoint of the gradient, assuming Neumann boundary conditions:
 %
%\begin{align}
%&\int_{\M} \mathrm{div}_{\M}V \phi \  dx  = - \int_{\M} g(V,\nabla_M{\phi}) \  dx\,.
%&div_{\M}(V) = -\int_{\mathcal{T}\M}\frac{1}{\sqrt{det g }}  \sum_i\frac{\partial V }{\partial x_i}\sqrt{det g } 
%\end{align}
%
 %
\begin{align}
&\int_{\M}  \mathrm{div}_{\M}V f  \  dx  = - \int_{\M} \langle V,\nabla_\M f \rangle_p \  dx\,,
\end{align}
%
where $f:\M\to\mathbb{R}$ is a scalar function and $V:\M\to\mathcal{T}\M$ is a vector field tangent to the surface.
%
In the following, to simplify the notation we will drop the subscript $\M$ whenever clear from the context.
%
We further denote by $\mathcal{L}^p(\M)=\{ f:\M\to\mathbb{R} ~| \int_\M |f(x)|^p dx <\infty\,, p\ge 1 \}$ the function space of $p$-integrable functions on $\M$.


\subsection{Total Variation}
%
%Let $f$  be a differentiable function on $\M$. Its total variation energy can be defined as:
 The total variation of a differentiable function $f$ on $\M$ is defined as
%
\begin{align} \label{mth:gradtv}
TV(f)=\int_{\M} \| \nabla f(x) \| dx  \,,
\end{align} 
%
where $\|\cdot\|$ is the norm induced by the inner product $\langle \cdot,\cdot\rangle_p$.
%
\sout{The total variation is a} \textcolor{red}{This} functional \sout{that} quantifies the amount of oscillations in a given signal. To account for non-differentiability of $f$, we adopt a weaker definition of TV  %In the case of non-differentiable functions $f \in \mathcal{L}^1(\M)$, we resort to a weak definition of the total variation
 in terms of continuously differentiable test vector fields $U:\M\to\mathcal{T}\M$ \cite{benartzi:2006}: %functions $\phi \in C_c^1(\M)$:
%
%\begin{align} \label{dfn:dualTV}
%    TV(f)=\sup_\phi\left\{ \int_ {\M} f(x) \mathrm{div} \phi(x) ~  dx :  ~ |\phi|_{\mathcal{L}^\infty(\mathcal{T}\M)}\leq 1\right\} \,.
%\end{align}
%
\begin{align} \label{dfn:dualTV}
    TV(f)=\sup_U\left\{ \int_ {\M} f(x) ~ \mathrm{div} U(x) \,  dx :  ~ \|U(x)\|\leq 1, ~ \forall x \right\} \,.
\end{align}
%
%For functions in $\mathcal{L}^1(\M)$, the energy is
Alternatively, one can define an \emph{anisotropic} variant of the standard TV by considering $U(x)$ to be bounded in the $L^\infty$ norm. We refer to functions $f$ of bounded variation, i.e. $TV(f)< +\infty$, to be in $BV(\M)$.

%The TV functional is absolutely one-homogeneous, i.e., $TV(sf)=|s|TV(f)$ for any $s\in\mathbb{R}$, and it is convex, therefore amenable to efficient optimization.
 
The TV functional is related to  fundamental geometric notions such as the curvature of level sets of a function, through the celebrated co-area formula \cite{Fleming:1960}. One particular case of this relation concerns the total variation of indicator functions of closed sets; in this case, the TV corresponds to the perimeter of the set (see \cite[Sec. 1.3]{chambolle:2010} for the Euclidean setting), which generalizes to manifolds in a straight forward way:
%
\begin{thm} \label{th:perimeter}
Let E $\subset \M$ be a measurable closed subset of $\M$, with smooth boundary $\partial E$, and let $\chi_E$ be its indicator function. Then:
\begin{align}
    %TV(\chi_E)=\int_{\M}||\nabla \chi_E|| dx= \mathrm{length}(\partial E)\,.
    TV(\chi_E)= \mathrm{length}(\partial E)\,.
\end{align}
\end{thm}
%
\noindent{\em Proof}: See Appendix \ref{apx:tper}.

\vspace{1ex}
As we show next, this particular class of indicator functions includes the set of generalized eigenfunctions of the operator associated to the TV functional.


==> Spectral TV (Copy)(3)/sections/related.tex <==
\section{Related Work}

From a general perspective, ours is a {\em filtering} approach that incorporates an edge-preserving diffusion process within a spectral decomposition framework, and draws inspiration from recent progress in nonlinear image processing. % including recent relevant literature from the field of nonlinear image processing.
In the following, we cover the works that more closely relate with these themes. 

\subsection{Variational mesh processing}
%
Our methodology falls within the class of energy minimization methods for geometry processing, and carries a natural dual interpretation as a diffusion-based approach. % some important analogies with diffusion-based approaches.

\vspace{1ex}\noindent\textbf{Diffusion-based methods.}
%
Following the work of Taubin \shortcite{Taubin:1995}, classical editing tasks such as surface smoothing, denoising and enhancement have been traditionally phrased as variants of the diffusion PDE $\partial_t u = \Delta_\mathcal{M} u$. Here, $u$ is a signal defined on the surface $\mathcal{M}$ \sout{(e.g., the vertex or normal coordinates for each point)}, and $\Delta_\mathcal{M}$ is its Laplace-Beltrami operator. For example, feature-aware denoising driven by local curvature has been addressed by modifying the metric on $\mathcal{M}$ (and hence its Laplacian), leading to a rich production of anisotropic techniques \cite{DMSB-gi2000,tasdizen2002geometric,Clarenz:2002,bajaj03}. Higher-order filtering with volume preservation to prevent surface shrinking was proposed in \cite{Desbrun:1999}; the same work clarified the well known duality relating the diffusion to mean curvature flow, and showed how the latter notion leads to \sout{an alternative and} a more robust formulation for denoising applications. This was later modified in \cite{kazhdan2012can} to resolve \sout{numerical} instabilities \sout{occurring across} of the flow. %\cite{Sorkine:2005} 

Our approach also involves a diffusion process, and comes with an associated geometric flow. 
%
We identify two key differences \textcolor{red}{over} \sout{as related to} prior work: (1) in our case, the operator involved is nonlinear, and (2) diffusion takes place {\em within} the level sets of the signal $u$ rather than {\em across} the boundary of the level sets. As a consequence, discontinuities are not smeared throughout the diffusion process, while contrast is reduced. In the inset figure, the source signal (left) is 
%
\setlength{\columnsep}{7pt}
\setlength{\intextsep}{3pt}
\begin{wrapfigure}{r}{0.45\linewidth}
\vspace{-0.15cm}
\begin{center}
\includegraphics[width=\linewidth]{images/smeared2.png}
%\input{./images/smeared.tex}
\end{center}
\end{wrapfigure}
%
processed via the classical ``horizontal'' isotropic diffusion (middle) and with our ``vertical'' diffusion (right); in the latter case, the \sout{step} width remains constant while the amplitude decreases. When the signal encodes surface geometry, this implies that sharp features are preserved. 


\vspace{1ex}\noindent\textbf{Energy minimization methods.}
%
%While diffusion-based methods often boil down to solving simple linear systems, their applicability is limited; % to a narrow class of geometric transformations. %
%in particular, 
Other approaches are based on formulating editing operations as the minimization of an energy. Although mathematically any variational \sout{minimization} problem can be rephrased as a diffusion problem, \sout{taking one of the two perspectives may be more or less convenient for computational reasons. Typically,} \sout{formulating a variational problem} choosing the former enables the implementation of a richer class of algorithms. 
%
%minimization enable a richer class of editing operations than diffusion-based techniques. Typically, 
%
Such methods lift ideas from \sout{the} image processing \sout{area} to the surface domain. For example, in \cite{He:2013} mesh denoising is done by minimizing the $L_0$ gradient norm of the vertex positions, thus suppressing low-amplitude details, as done in \cite{xu:2011} for images; extensions to meshes of bilateral \cite{tomasi:1998} and mean shift \cite{meanshift} filtering were proposed in  \cite{fleishman03,Solomon:2014}\sout{ respectively}; \textcolor{red}{a variant of \cite{Zhang_rolling:2014} was applied to the normal vector field in \cite{wang:2015}}; \sout{more recently,} shock filters \cite{shock90} were applied to surface geometry for feature sharpening and enhancement in \cite{Prada:2015}. Gradient-domain mesh processing \cite{Chuang:2016:GPO} is also a recent direction inspired by success in the image domain, allowing explicit prescription of target gradient fields.\sout{ Other filtering methods allow prescribing vertex positions \cite{kobbelt98,Sorkine:2005} or the Riemannian metric directly \cite{chuang:2011}.} %, vertex positions  or Riemannian metric  have also been proposed.


The above testifies to a wealthy literature of nonlinear edge preserving strategies for mesh filtering. The main drawback of these methods lies in their lack of generality. Here we provide a general framework to perform multiscale analysis and synthesis of arbitrary signals defined on geometric domains (meshes and point clouds alike); while denoising, fairing and enhancement can be easily realized within this framework, we are not limited to these applications and provide a more flexible setting for geometry processing.

\vspace{1ex}\noindent\textbf{TV-based methods.}
%
\sout{Ours is certainly not the first work to consider the total variation functional in a geometry processing context.} TV and the strictly related Mumford-Shah functional have been considered before for different tasks in geometry processing, \textcolor{red}{e.g. surface reconstruction \cite{Liu:2017}}. % of mesh denoising \cite{Zhang:2015,Zhong:2018}, feature line detection \cite{Tong:2016}, inpainting and segmentation \cite{Bonneel:2018} among others. 
%
 Zhang et al.~\shortcite{Zhang:2015} consider an extension of the ROF model \cite{Rudin:1992} for denoising surfaces, which they solve with an augmented Lagrangian method followed by a geometry reconstruction step \cite{Sun:2007}. Zhong et al.~\shortcite{Zhong:2018} follow a similar approach, with the inclusion of an additional regularizer defined as the Laplacian energy of the normal coordinates, which helps dampen the staircase effect that is observed in \cite{Zhang:2015}.
% 
\sout{The resulting energy is also minimized as in Zhang 2015.}
%
These methods are related to ours, \sout{since} as they \sout{both} involve the minimization of the TV of the surface normal field; we also consider this kind of energy, but in addition, we study the {\em geometric flow} associated to it. Further, our approach is not restricted to normal fields, but allows processing arbitrary surface signals\sout{ defined on the surface}. Tong and Tai~\shortcite{Tong:2016} consider the Mumford-Shah functional \sout{, instead of the TV functional,} as a measure of sharp geometric variation for a given signal. Their focus is on the detection of features lines (i.e. the boundaries between neighboring segments) for scalar functions such as mean curvature and color texture, rather than geometry processing. The \sout{Mumford-Shah} MS functional has also been considered in \cite{Bonneel:2018} in its Ambrosio-Tortorelli approximation. The authors extend the range of possible applications of \cite{Tong:2016} by operating on the surface normal field, showing results in  inpainting, denoising and segmentation tasks. In addition to lacking an analysis of the TV normal flow, none of these methods provide a {\em spectral} framework based on the TV functional for geometry processing.
\subsection{Spectral geometry processing}
%
%An important distinction with prior multiresolution schemes for mesh filtering \cite{kobbelt98,guskov99}, which are typically formulated as sequences of downsampling steps, 
As shown in Figure~\ref{fig:teaser}, our multiscale approach provides a sharp separation of an input signal into ``feature bands''. %\MM{Fig. 1 does not really illustrate feature bands, does it?}
%
We achieve this by means of a generalized {\em spectral} decomposition. Spectral geometry processing was introduced \sout{again} by \sout{the work of} Taubin~\shortcite{Taubin:1995} and further developed in \cite{Sorkine:2005,Levy:2006,rong2008spectral,Zhang:2010} for tasks of shape reconstruction, modelling, and deformation transfer among others. These works generalize Fourier analysis to 
%
\setlength{\columnsep}{7pt}
\setlength{\intextsep}{1pt}
\begin{wrapfigure}[6]{r}{0.55\linewidth}
\vspace{-0.15cm}
\begin{center}
\begin{overpic}
[trim=0cm 0cm 0cm 0cm,clip,width=1.0\linewidth]{./images/gibbs2.png}
\vspace{0.1cm}
\put(2.5,-20.8){\frame{\includegraphics[width=0.25\linewidth]{plot1.png}}}
\put(33.5,-20.8){\frame{\includegraphics[width=0.25\linewidth]{plot2.png}}}
\put(64.5,-20.8){\frame{\includegraphics[width=0.25\linewidth]{plot3.png}}}
\end{overpic}
\end{center}
\end{wrapfigure}
%\sout{These methods leverage several key properties of the Laplacian: it is isometry invariant (thus fully intrinsic), easy to compute on meshes and point clouds, and its}
%
  surfaces by observing that the Laplacian eigenvectors form an orthogonal set of smooth basis functions with a canonical ordering (low to high frequencies). This basis is optimal for representing smooth functions compactly \cite{Aflalo:2014}, but it gives rise to \sout{undesirable} artifacts in the presence of sharp variations, thus \sout{greatly} reducing the benefits of working with a spectral representation; in the inset, we show the typical blurring effect (middle) and Gibbs oscillations (right) due to the \sout{presence of} jumps in the source signal (left), \sout{which are} not handled well by the smooth Laplacian eigenbasis.

%
Variants of the Laplace operator \sout{have been considered in order to} add flexibility and \sout{incorporate} feature awareness\sout{ in the spectral basis}, including anisotropic \cite{Andreux:2015} and extrinsic \cite{Liu:2017} variants, see \cite{Wang:2019} for a recent survey. Sparsity \sout{in the context of spectral geometry} has \sout{also} been analyzed in \cite{Neumann:2014}, where Laplacian eigenfunctions are modified to have limited support by penalizing their $L^1$ norm. We differ in that we consider signals with sparse gradients instead.  %An ad-hoc basis for piecewise-constant functions was also proposed \cite{MELZI2019117}, although at the cost of losing the aforementioned benefits of spectral representations.
%
 \sout{Despite recent progress,} All these operators are linear, and their associated energies promote smoothness\sout{ (we formalize this statement more precisely below)}. Our operator is nonlinear, hence more powerful, and its \sout{(generalized)} eigenfunctions are well suited to represent jump discontinuities in the signal. This yields a cleaner separation of different features into different bands, \sout{; this is} in contrast to Laplacian-based representations, which spread individual features across the entire spectrum.

%Moreover, our signal decomposition is driven by the data: 

%We inspect a spectral, data-driven representation based on this operator for the first time on surfaces. 

%are typically addressed by either modifying the metric underlying the definition of the operator \cite{Andreux:2015,schonsheck2018nonisometric}, or by ex-post refinement \cite{marin2019cmh}.

%


\subsection{Nonlinear image processing}
%
%Similarly to previous successful research in geometry processing \cite{}, in this work we adopt tools from the image processing area while bringing them to the non-Euclidean setting.
%
Finally, similar to prior research, our approach is also based on ideas originating from image processing.
%
In this field, nonlinear variational methods have replaced linear methods due to their higher precision in approximating natural phenomena. To date, a major role has been played by the total variation (TV) energy and its minimization, originally exploited by Rudin et al.~\shortcite{Rudin:1992} with the ROF model for image denoising. Other uses of the TV functional span image deblurring, inpainting, interpolation, image decomposition, super-resolution and stereovision, to name but a few; for a general introduction to the topic see \cite{chambolle:2010}.
%
Recently, a spectral theory related to the gradient flow of this functional (c.f. Bellettini et al.~\shortcite{bellettini:2002}) on eigenfunctions, was developed by Gilboa \shortcite{Gilboa:2013,GuySpectralSiam14} and generalized in \cite{Gilboa:2015, Burger:2016} with applications to image processing, allowing for the analysis of images at different scales by exploiting the edge-preserving property of the total variation. Here we propose to lift this latter framework from the Euclidean domain to surfaces, put it in relation to existing geometry processing models, and demonstrate several possible applications in the area of 3D graphics.

%The motivations comes from applications in the image processing community where the total variation has been widely exploited as a regularizing energy for solving several classes of problems, leveraging on its property to promote signals with sparse gradient and the consequent preservation of discontinuities (edges) in the image, which represent object contours. 
%The typical setting is to solve an inverse, ill posed problem, exploiting priors on the signals to make the problem tractable. One such priors is indeed the total variation functional which allows to act on an input image at different scales, while allowing to recover the edges of objects in the image. 
%We show here that all the desirable properties of this functional can be lifted from the Euclidean domain to curved surfaces. 
%Moreover, through the analysis of the spectrum of the related operator, we show that is possible to define a transform which allows to obtain a sparse representation of functions defined on surfaces providing a way to analyze possibly discontinuous functions at different scales. 






%-----------------------------------------
\begin{comment}


\subsection{Euclidean Domains}

In the image processing field the total variation has served as a prior to reconstruct signals while preserving the edges of the image, following the fashion of nonlinear filters based on variational methods. The minimization of this functional, originally exploited by Rudin et al \cite{Rudin:1992} in their ROF model for image denoising, has proven extremely useful for many applications which spans from image deblurring, inpainting, interpolation, to spectral extrapolation, image decomposition, super-resolution, stereovision, and much more. For a good introduction to the topic see \cite{chambolle:2010}.
In particular Gilboa et al \cite{Gilboa:2013,Gilboa:2015} recently developed a spectral theory related to this functional which enables to obtain a new representation of images at different scales exploiting the discontinuities preservation property of the total variation. 

\subsection{Surfaces}
Spectral approaches on surfaces are typically related to the eigendecomposition of the Laplace Beltrami operator, which generalizes Fourier analysis on signals defined on manifolds. While others operators have been considered to overcome certain limitations (see \cite{Wang:2019} for a complete survey), nonlinear alternatives have not been paid much attention. 

The total variation functional itself has found few applications in geometry processing, compared to its use in image processing, and has been exploited only as a regularization term in some particular settings, mainly denoising of models through filtering of surface normals \cite{Zhang:2015}.
Following approaches like \cite{Prada:2015}, we propose to lift aspects analyzed in image processing field to surface domains providing a new way to analyze functions on manifolds, which relies on a solid mathematical theory. %We present the first spectral approach to total variation on surfaces.
\end{comment}

==> images/plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
%\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor1}{rgb}{1.00000,0.5882,0}%
%
\begin{tikzpicture}%
\begin{axis}[%
width=0.20\linewidth,
height=0.20\linewidth,
at={(-5.5cm,0)},
scale only axis,
ytick={0, 1},
yticklabels={0, 1},
xtick={0,1,3,5},
xticklabels={t=,1,3,5},
every x tick label/.append style={font=\color{black}, font=\footnotesize},
every y tick label/.append style={font=\color{black}, font=\tiny},
%xlabel={\footnotesize $t$},
ylabel={\footnotesize $u(t)$},
ylabel style={yshift=-0.25cm},
xlabel style={yshift=0.1cm},
xmin=0,
xmax=6,
ymin=-0.1,
ymax=1.2,
axis background/.style={fill=white}
]%
\addplot[forget plot, color=white!15!gray, dotted, line width=0.9pt] table[row sep=crcr] {%
0	0\\
6	0\\
};%
\addplot [color=mycolor1, line width=1.5pt, forget plot]%
  table[row sep=crcr]{%
0	1\\
0.00600600600600601	0.997998198198198\\
0.012012012012012	0.995996396396396\\
2.99099099099099	0.00310270270270274\\
2.996996996997	0.00110090090090087\\
3.003003003003	0\\
3.00900900900901	0\\
5.99399399399399	0\\
6	0\\
};%
\end{axis}%
\begin{axis}[%
width=0.20\linewidth,
height=0.20\linewidth,
at={(-2.75cm,0)},
%xlabel={ \footnotesize $t$},
ylabel={\footnotesize $\partial_t u(t)$},
ylabel style={yshift=-0.4cm},
ytick={-0.33, 0},
%ytick={-0.4, -0.3, -0.2, -0.1,    0,  0.1,  0.2},
yticklabels={-1/3,},
xtick={0,1,3,5},
xticklabels={t=,1,3,5},
every x tick label/.append style={font=\color{black}, font=\footnotesize},
xlabel style={yshift=0.05cm},
every y tick label/.append style={font=\color{black}, font=\tiny},
scale only axis,
xmin=0,
xmax=6,
ymin=-0.4,
ymax=0.2,
axis background/.style={fill=white}
]%
\addplot[forget plot, color=white!15!gray, dotted, line width=0.9pt] table[row sep=crcr] {%
0	0\\
6	0\\
};%
\addplot [color=mycolor1, line width=1.5pt, forget plot]%
  table[row sep=crcr]{%
0	-0.3333\\
0.00600600600600601	-0.3333\\
2.94294294294294	-0.3333\\
2.98498498498498	-0.3333\\
2.99099099099099	-0.3333\\
2.996996996997	-0.3333\\
3.003003003003	0\\
3.00900900900901	0\\
3.08108108108108	0\\
6	0\\
};%
\end{axis}%
\begin{axis}[%
width=0.20\linewidth,
height=0.20\linewidth,
%xlabel={ \footnotesize $t$},
ylabel={\footnotesize $\partial_{tt} u(t)$},
ylabel style={yshift=-0.25cm},
ytick={0, 1},
yticklabels={0, 1},
xtick={0,1,3,5},
xticklabels={t=,1,3,5},
every x tick label/.append style={font=\color{black}, font=\footnotesize},
xlabel style={yshift=0.05cm},
every y tick label/.append style={font=\color{black}, font=\tiny},
scale only axis,
xmin=0,
xmax=6,
ymin=-0.1,
ymax=1.2,
axis background/.style={fill=white}
]%
\addplot[ycomb, color=mycolor1, line width=1.5pt, mark=triangle, mark options={solid, mycolor1}, forget plot] table[row sep=crcr] {%
3.000300030003	1\\
};%
\addplot[forget plot, color=white!15!gray, dotted, line width=0.9pt] table[row sep=crcr] {%
0	0\\
6	0\\
};%
\node[right, align=left]
at (axis cs:3.2,1) {$\infty$};
\end{axis}%
\end{tikzpicture}%

==> images/plottt.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(9.926in,0.596in)},
scale only axis,
xmin=0,
xmax=3,
ymin=0,
ymax=50,
xlabel=${t}$,
ylabel=$S(t)$,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	0\\
0.12	0\\
0.18	0\\
0.24	0\\
0.3	0\\
0.36	0\\
0.42	0\\
0.48	0\\
0.54	0\\
0.6	0\\
0.66	0\\
0.72	0\\
0.78	0\\
0.84	0\\
0.9	0\\
0.96	0\\
1.02	0\\
1.08	0\\
1.14	0\\
1.2	0\\
1.26	0\\
1.32	0\\
1.38	0\\
1.44	0\\
1.5	0\\
1.56	0\\
1.62	1.61326896783028\\
1.68	10.8664542039284\\
1.74	14.8863609697787\\
1.8	7.63896040637369\\
1.86	0.582923459225431\\
1.92	0\\
1.98	0\\
2.04	0\\
2.1	0\\
2.16	0\\
2.22	0\\
2.28	0\\
2.34	0\\
2.4	0\\
2.46	0\\
2.52	0\\
2.58	0\\
2.64	0\\
2.7	0\\
2.76	0\\
2.82	0\\
2.88	0\\
2.94	0\\
3	0\\
};
\end{axis}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(7.192in,0.596in)},
scale only axis,
xmin=0,
xmax=3,
ymin=0,
xlabel=${t}$,
ylabel=$S(t)$,
ymax=50,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	0\\
0.12	0\\
0.18	0\\
0.24	0\\
0.3	0\\
0.36	0\\
0.42	0\\
0.48	0\\
0.54	0\\
0.6	0\\
0.66	0\\
0.72	0\\
0.78	0\\
0.84	0\\
0.9	0\\
0.96	0\\
1.02	0\\
1.08	0\\
1.14	0\\
1.2	8.33793739352754\\
1.26	26.0897929810706\\
1.32	23.1722162857857\\
1.38	9.34430416355465\\
1.44	0\\
1.5	0\\
1.56	0\\
1.62	0\\
1.68	0\\
1.74	0\\
1.8	0\\
1.86	0\\
1.92	0\\
1.98	0\\
2.04	0\\
2.1	0\\
2.16	0\\
2.22	0\\
2.28	0\\
2.34	0\\
2.4	0\\
2.46	0\\
2.52	0\\
2.58	0\\
2.64	0\\
2.7	0\\
2.76	0\\
2.82	0\\
2.88	0\\
2.94	0\\
3	0\\
};
\end{axis}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(4.458in,0.596in)},
scale only axis,
xmin=0,
xlabel=${t}$,
ylabel=$S(t)$,
xmax=3,
ymin=0,
ymax=50,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	0\\
0.12	0\\
0.18	0\\
0.24	0\\
0.3	0\\
0.36	0\\
0.42	0\\
0.48	0\\
0.54	0\\
0.6	0\\
0.66	0\\
0.72	0\\
0.78	0\\
0.84	2.66365572617013\\
0.9	2.61165782452093\\
0.96	16.4075476525552\\
1.02	42.1779801784895\\
1.08	24.1490851884908\\
1.14	0\\
1.2	0\\
1.26	0\\
1.32	0\\
1.38	0\\
1.44	0\\
1.5	0\\
1.56	0\\
1.62	0\\
1.68	0\\
1.74	0\\
1.8	0\\
1.86	0\\
1.92	0\\
1.98	0\\
2.04	0\\
2.1	0\\
2.16	0\\
2.22	0\\
2.28	0\\
2.34	0\\
2.4	0\\
2.46	0\\
2.52	0\\
2.58	0\\
2.64	0\\
2.7	0\\
2.76	0\\
2.82	0\\
2.88	0\\
2.94	0\\
3	0\\
};
\end{axis}

\begin{axis}[%
width=2.078in,
height=1.848in,
at={(1.724in,0.596in)},
scale only axis,
xmin=0,
xmax=3,
ymin=0,
ymax=50,
xlabel=${t}$,
ylabel=$S(t)$,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.06	1\\
0.12	0.0354221564742846\\
0.18	0.0836880769716178\\
0.24	0.238515084607873\\
0.3	0.42369682621709\\
0.36	0.294829775280522\\
0.42	0.249205370448056\\
0.48	0.44619627845989\\
0.54	1.13388529065136\\
0.6	1.06936269974406\\
0.66	0.485097844802714\\
0.72	1.25885192956809\\
0.78	2.53080986474693\\
0.84	2.66365572617013\\
0.9	2.61165782452093\\
0.96	16.4075476525552\\
1.02	42.1779801784895\\
1.08	24.1490851884908\\
1.14	3.41464216740326\\
1.2	8.33793739352754\\
1.26	26.0897929810706\\
1.32	23.1722162857857\\
1.38	9.34430416355465\\
1.44	3.44171093089059\\
1.5	5.59118508341205\\
1.56	3.67877300861255\\
1.62	1.61326896783028\\
1.68	10.8664542039284\\
1.74	14.8863609697787\\
1.8	7.63896040637369\\
1.86	0.582923459225431\\
1.92	3.06471770053865\\
1.98	1.98939679353392\\
2.04	0.480183113497467\\
2.1	0.654214042504147\\
2.16	0.485439759045626\\
2.22	0.350683443571814\\
2.28	0.4174235136317\\
2.34	0.391300787515381\\
2.4	0.359935832863793\\
2.46	0.361220649315936\\
2.52	0.370039226720947\\
2.58	0.381070671319322\\
2.64	0.390812784387449\\
2.7	0.398571914814711\\
2.76	0.404053295448914\\
2.82	0.404623372677762\\
2.88	0.395091008572386\\
2.94	0.36869534607641\\
3	0.317572637938863\\
};
\end{axis}


\end{tikzpicture}%

==> images/smeared.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mygray}{rgb}{0.50000,0.5,0.5}%
\definecolor{myblue}{rgb}{0.0804,0.5898,1}%
%
\begin{tikzpicture}
%
\begin{axis}[%
width=0.3\linewidth,
height=0.16\linewidth,
scale only axis,
xmin=-1,
xmax=1,
ymin=-0.1,
ymax=1.1,
axis line style={draw=none},
ticks=none,
legend style={legend cell align=left, align=left, draw=white!15!black}%
]%
\addplot [color=black, line width=1.6pt, forget plot]%
  table[row sep=crcr]{%
-1	0\\
-0.507537688442211	0\\
-0.49748743718593	1\\
0.49748743718593	1\\
0.507537688442211	0\\
1	0\\
};%
%
\end{axis}
%
\begin{axis}[%
width=0.3\linewidth,
height=0.16\linewidth,
at={(1.3cm,0)},
scale only axis,
xmin=-1,
xmax=1,
ymin=-0.1,
ymax=1.1,
axis line style={draw=none},
ticks=none,
legend style={legend cell align=left, align=left, draw=white!15!black}%
]%
\addplot [color=myblue, line width=1.6pt, forget plot]%
  table[row sep=crcr]{%
-1	0.0124316567871479\\
-0.979899497487437	0.0130917512766948\\
-0.959798994974874	0.0146526292205273\\
-0.939698492462312	0.0171633294536573\\
-0.919597989949749	0.0206993584857882\\
-0.899497487437186	0.0253605768668288\\
-0.879396984924623	0.0312682533993369\\
-0.85929648241206	0.0385612508652649\\
-0.839195979899497	0.047391324424003\\
-0.829145728643216	0.0524323585697029\\
-0.819095477386935	0.0579175464022208\\
-0.809045226130653	0.0638668667771738\\
-0.798994974874372	0.0702999180241104\\
-0.78894472361809	0.0772356828790115\\
-0.778894472361809	0.0846922871047318\\
-0.768844221105528	0.0926867539082068\\
-0.758793969849246	0.101234756512811\\
-0.748743718592965	0.110350371472953\\
-0.738693467336683	0.120045835518684\\
-0.728643216080402	0.130331308883783\\
-0.718592964824121	0.141214648195071\\
-0.708542713567839	0.152701192077583\\
-0.698492462311558	0.164793562654784\\
-0.678391959798995	0.190791635232835\\
-0.658291457286432	0.219169268976531\\
-0.638190954773869	0.249834462032695\\
-0.618090452261307	0.282640967168752\\
-0.597989949748744	0.317388599998267\\
-0.577889447236181	0.353825824698808\\
-0.557788944723618	0.391654619044215\\
-0.527638190954774	0.450260085944638\\
-0.447236180904523	0.608345380955784\\
-0.42713567839196	0.646174175301191\\
-0.407035175879397	0.682611400001732\\
-0.386934673366834	0.717359032831246\\
-0.366834170854272	0.750165537967304\\
-0.346733668341709	0.780830731023469\\
-0.326633165829146	0.809208364767164\\
-0.306532663316583	0.835206437345215\\
-0.296482412060302	0.847298807922416\\
-0.28643216080402	0.858785351804927\\
-0.276381909547739	0.869668691116216\\
-0.266331658291457	0.879954164481315\\
-0.256281407035176	0.889649628527045\\
-0.246231155778895	0.898765243487187\\
-0.236180904522613	0.907313246091791\\
-0.226130653266332	0.915307712895266\\
-0.21608040201005	0.922764317120986\\
-0.206030150753769	0.929700081975887\\
-0.195979899497488	0.936133133222824\\
-0.185929648241206	0.942082453597777\\
-0.175879396984925	0.947567641430295\\
-0.155778894472362	0.957225688506778\\
-0.135678391959799	0.965267656676309\\
-0.115577889447236	0.971849709455752\\
-0.0954773869346734	0.977117798921691\\
-0.0753768844221105	0.981202522974995\\
-0.0552763819095479	0.984214868075998\\
-0.035175879396985	0.986242833013094\\
-0.0150753768844221	0.987348904251816\\
0.00502512562814061	0.987568343212849\\
0.0251256281407035	0.986908248723303\\
0.0452261306532664	0.98534737077947\\
0.0653266331658291	0.98283667054634\\
0.085427135678392	0.979300641514209\\
0.105527638190955	0.974639423133169\\
0.125628140703518	0.968731746600661\\
0.14572864321608	0.961438749134733\\
0.165829145728643	0.952608675575995\\
0.175879396984925	0.947567641430295\\
0.185929648241206	0.942082453597777\\
0.195979899497488	0.936133133222824\\
0.206030150753769	0.929700081975887\\
0.21608040201005	0.922764317120986\\
0.226130653266332	0.915307712895266\\
0.236180904522613	0.907313246091791\\
0.246231155778895	0.898765243487188\\
0.256281407035176	0.889649628527045\\
0.266331658291457	0.879954164481315\\
0.276381909547739	0.869668691116216\\
0.28643216080402	0.858785351804928\\
0.296482412060302	0.847298807922416\\
0.306532663316583	0.835206437345215\\
0.326633165829146	0.809208364767164\\
0.346733668341709	0.780830731023469\\
0.366834170854271	0.750165537967304\\
0.386934673366834	0.717359032831247\\
0.407035175879397	0.682611400001732\\
0.42713567839196	0.646174175301191\\
0.447236180904523	0.608345380955784\\
0.477386934673367	0.54973991405536\\
0.557788944723618	0.391654619044215\\
0.577889447236181	0.353825824698808\\
0.597989949748744	0.317388599998267\\
0.618090452261306	0.282640967168752\\
0.638190954773869	0.249834462032695\\
0.658291457286432	0.21916926897653\\
0.678391959798995	0.190791635232835\\
0.698492462311558	0.164793562654784\\
0.708542713567839	0.152701192077583\\
0.71859296482412	0.141214648195071\\
0.728643216080402	0.130331308883783\\
0.738693467336683	0.120045835518684\\
0.748743718592965	0.110350371472953\\
0.758793969849246	0.101234756512811\\
0.768844221105528	0.0926867539082068\\
0.778894472361809	0.0846922871047318\\
0.78894472361809	0.0772356828790115\\
0.798994974874372	0.0702999180241104\\
0.809045226130653	0.0638668667771738\\
0.819095477386935	0.0579175464022208\\
0.829145728643216	0.0524323585697029\\
0.849246231155779	0.0427743114932193\\
0.869346733668342	0.0347323433236881\\
0.889447236180904	0.0281502905442457\\
0.909547738693467	0.022882201078307\\
0.92964824120603	0.0187974770250026\\
0.949748743718593	0.0157851319239992\\
0.969849246231156	0.013757166986903\\
0.989949748743719	0.0126510957481811\\
1	0.0124316567871479\\
};
%
\draw[-{Stealth[scale=1.1,inset=1.8pt,angle=90:10pt,color=gray,width=1.6mm,length=1.8mm]},semithick,gray] (-0.55,0.35) -- (0.55,0.35);
\draw[-{Stealth[scale=1.1,inset=1.8pt,angle=90:10pt,color=gray,width=1.6mm,length=1.8mm]},semithick,gray] (0.55,0.35) -- (-0.55,0.35);
%
\end{axis}
%
\begin{axis}[%
width=0.3\linewidth,
height=0.16\linewidth,
at={(2.6cm,0)},
scale only axis,
xmin=-1,
xmax=1,
ymin=-0.1,
ymax=1,
axis line style={draw=none},
ticks=none,
legend style={legend cell align=left, align=left, draw=white!15!black}%
]%
\addplot [color=myblue, line width=1.6pt, forget plot]%
  table[row sep=crcr]{%
-1	0\\
-0.507537688442211	0\\
-0.49748743718593	0.4\\
0.49748743718593	0.4\\
0.507537688442211	0\\
1	0\\
};%
\draw[-{Stealth[scale=1.1,inset=1.8pt,angle=90:10pt,color=gray,width=1.6mm,length=1.8mm]},semithick,gray] (0,1) -- (0,0.4);
%
\end{axis}
%
%
\end{tikzpicture}%

==> images/treeplot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}
\begin{axis}[%
width=0.5\linewidth,
height=0.4\linewidth,
scale only axis,
xmajorgrids=true,
ymajorgrids=true,
every x tick label/.append style={font=\color{black}, font=\tiny},
every y tick label/.append style={font=\color{black}, font=\tiny},
ylabel style={yshift=-0.27cm},
ylabel style={xshift=-0.15cm},
xlabel style={yshift=0.17cm},
xmin=0,
xmax=3000,
xtick={0,1000,2000,3000},
xticklabels={0,1,2,3},
ytick={0,5000,10000},
yticklabels={0,,1},
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize Iteration ($\times 10^3$)},
ymin=0,
ymax=12000,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize TV energy},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={TV energy},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	8769.80567714888\\
3	8765.52060208535\\
6	8753.19870636316\\
10	8727.66111430032\\
15	8682.22208927593\\
21	8611.1679283053\\
30	8482.56228064604\\
47	8231.84418580489\\
73	7870.65280914336\\
91	7589.58614637022\\
117	7176.29431066304\\
127	7054.77059223718\\
140	6918.18548347215\\
175	6580.34393422045\\
188	6473.82821942617\\
215	6306.79157750887\\
226	6220.46841590536\\
236	6130.85882474641\\
249	6012.92683989099\\
260	5933.13604772369\\
266	5902.2598691463\\
286	5806.35904188635\\
296	5749.15997915603\\
314	5641.54918417365\\
345	5490.70561114222\\
355	5439.91918205179\\
367	5369.13998040854\\
387	5250.76948646463\\
399	5191.7422425948\\
414	5130.8492403156\\
426	5081.23042860648\\
463	4912.62785223861\\
471	4880.4776548674\\
481	4848.0619223422\\
494	4810.64507490459\\
508	4767.93847885284\\
519	4727.61524389073\\
550	4610.96550241506\\
557	4591.51193073569\\
567	4569.77743586156\\
591	4517.70972596239\\
609	4469.90139254135\\
628	4423.54846674126\\
648	4369.07492801303\\
677	4299.94310190137\\
682	4292.62112315639\\
691	4283.94144730481\\
701	4273.80408713521\\
720	4249.65352683481\\
732	4229.49252045151\\
748	4198.861309599\\
772	4146.23760459513\\
783	4122.15991394254\\
798	4092.73150577211\\
808	4068.01082555487\\
818	4038.35674322214\\
833	3987.40456568868\\
861	3879.95976558432\\
897	3745.50869204234\\
907	3716.44208462268\\
944	3627.41436387601\\
956	3591.75281018165\\
1000	3454.54209605356\\
1019	3403.79006415259\\
1039	3351.55111301218\\
1052	3312.02909201736\\
1071	3248.42261924547\\
1106	3128.77900846884\\
1113	3109.61331215802\\
1122	3091.27907023858\\
1136	3067.54776433203\\
1146	3053.55677953313\\
1155	3043.02032076248\\
1174	3022.79067289064\\
1209	2984.35951391489\\
1236	2945.70315345639\\
1259	2914.85047604769\\
1274	2894.34090030341\\
1293	2864.8364468102\\
1304	2848.9213213193\\
1321	2827.4305856946\\
1337	2807.47858652667\\
1350	2790.47637742014\\
1374	2765.0419230003\\
1384	2758.08015912145\\
1395	2752.17369725413\\
1403	2749.3970023681\\
1418	2744.74735744541\\
1426	2740.41932582834\\
1434	2733.93432471629\\
1442	2725.21744713767\\
1456	2706.47310609922\\
1480	2669.87699963885\\
1519	2605.4500996022\\
1548	2555.67374708552\\
1557	2544.5148062697\\
1566	2535.82702222485\\
1593	2514.54710694349\\
1602	2509.15521265019\\
1611	2505.73472131211\\
1619	2504.32144220168\\
1623	2505.15465380309\\
1636	2512.12597173624\\
1649	2517.96207204616\\
1670	2524.78404040088\\
1682	2526.34942406507\\
1697	2525.8474411031\\
1741	2521.55637672356\\
1761	2517.86695362734\\
1770	2513.39868070206\\
1779	2506.95550134922\\
1791	2495.90215132068\\
1830	2457.81727984579\\
1847	2441.31490656497\\
1867	2419.1369178171\\
1901	2381.00850024565\\
1921	2363.85352414888\\
1957	2335.53689928676\\
1963	2332.67572944614\\
1970	2331.17012275184\\
1979	2331.3986295762\\
2005	2333.98660748028\\
2024	2336.91933050283\\
2044	2340.14780063025\\
2065	2341.5292648391\\
2077	2340.46300584343\\
2090	2337.49786964739\\
2105	2331.76264729285\\
2166	2305.8037800657\\
2186	2300.36596434554\\
2222	2291.33805232033\\
2240	2283.77398112982\\
2256	2275.3927150391\\
2275	2262.87275449203\\
2297	2248.08989979396\\
2309	2242.15167615458\\
2332	2232.97669713028\\
2351	2224.77187911786\\
2364	2216.88876433548\\
2378	2206.06664404491\\
2404	2184.95588643737\\
2416	2177.29457953881\\
2463	2151.7182628464\\
2515	2127.27728830258\\
2535	2121.39195303474\\
2562	2114.55071084212\\
2578	2108.58621884492\\
2628	2087.94401443079\\
2651	2080.25598812873\\
2681	2071.09839012658\\
2701	2063.68138780557\\
2718	2055.58134480964\\
2745	2042.59158472335\\
2823	2008.67422338832\\
2839	1999.19300789203\\
2867	1982.38551697393\\
2889	1970.95692753235\\
2915	1959.59875683782\\
2951	1945.5664755403\\
2970	1939.80677396461\\
2991	1935.22020298349\\
2999	1933.84099657846\\
};
\addlegendentry{\footnotesize original}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	10282.0899593612\\
3	10240.8393369436\\
6	10125.466637058\\
10	9889.64524134536\\
16	9422.42888787062\\
28	8309.26230309407\\
39	7352.78915583833\\
50	6532.01735473021\\
62	5790.63661668084\\
80	4776.52254977473\\
89	4359.38492374121\\
96	4102.16732395772\\
107	3787.71059811782\\
118	3503.17106460966\\
126	3333.09489468827\\
131	3259.45367840321\\
135	3223.76848756533\\
138	3209.78813963662\\
141	3203.39382823318\\
154	3186.84011282525\\
162	3169.83785127707\\
180	3117.2572258599\\
184	3108.40364712658\\
191	3087.3562934762\\
198	3062.88621623496\\
204	3043.95045311897\\
224	2989.34078398757\\
231	2962.66956346121\\
238	2926.37221018255\\
253	2839.94192202754\\
267	2749.66071420537\\
279	2656.37391623455\\
307	2439.80630538242\\
322	2343.53041372188\\
330	2300.65424195822\\
340	2257.2994396219\\
349	2225.85037066919\\
358	2200.14958907804\\
368	2172.18233501462\\
383	2130.7338196834\\
390	2117.25996004967\\
431	2047.78242841884\\
437	2041.56194343109\\
450	2032.72105311146\\
476	2018.21626552898\\
483	2011.98182420321\\
489	2004.65188377867\\
496	1992.71960959904\\
504	1975.3168186967\\
522	1933.13963414107\\
545	1888.46892964927\\
556	1871.01303124894\\
566	1858.12849886948\\
580	1843.17403824954\\
588	1837.23855009064\\
599	1832.45144175262\\
614	1826.35197991301\\
641	1812.89249923677\\
653	1810.1313947828\\
664	1807.6828551932\\
672	1803.9879310629\\
681	1797.23946420362\\
702	1779.98251640605\\
712	1775.22782167409\\
723	1769.40903929834\\
733	1762.18339036431\\
744	1751.62346068541\\
771	1723.74524671412\\
782	1715.47151818146\\
793	1709.13617044166\\
802	1706.02023590914\\
815	1703.25767567192\\
880	1691.14126089583\\
911	1683.38975071214\\
929	1678.98366437674\\
953	1670.92914465903\\
974	1664.88040949725\\
1028	1649.71431451163\\
1073	1632.3601954541\\
1087	1629.11104696314\\
1102	1627.47999581991\\
1139	1624.27387252886\\
1172	1618.3197000878\\
1223	1606.99623914085\\
1251	1604.26034770985\\
1271	1603.74894491219\\
1305	1603.03117957847\\
1329	1601.1453996877\\
1355	1597.07549565886\\
1448	1580.68185897398\\
1480	1579.04357642985\\
1540	1576.05469636721\\
1584	1572.46436947919\\
1647	1567.64365305155\\
2037	1554.86004024981\\
2121	1553.58495724715\\
2214	1552.74730190819\\
2270	1551.51420469486\\
2407	1547.47944144937\\
2494	1544.81557924314\\
2559	1543.58033556663\\
2948	1541.57011783912\\
};
\addlegendentry{\footnotesize intrinsic triang}
\legend{}
\end{axis}
\end{tikzpicture}%
